Wide and Deep Neural Networks Achieve Optimality for Classification

While neural networks are used for classification tasks across domains, a long-standing open problem in machine learning is determining whether neural networks trained using standard procedures are optimal for classification, i.e., whether such models minimize the probability of misclassification for arbitrary data distributions. In this work, we identify and construct an explicit set of neural network classifiers that achieve optimality. Since effective neural networks in practice are typically both wide and deep, we analyze infinitely wide networks that are also infinitely deep. In particular, using the recent connection between infinitely wide neural networks and Neural Tangent Kernels, we provide explicit activation functions that can be used to construct networks that achieve optimality. Interestingly, these activation functions are simple and easy to implement, yet differ from commonly used activations such as ReLU or sigmoid. More generally, we create a taxonomy of infinitely wide and deep networks and show that these models implement one of three well-known classifiers depending on the activation function used: (1) 1-nearest neighbor (model predictions are given by the label of the nearest training example); (2) majority vote (model predictions are given by the label of the class with greatest representation in the training set); or (3) singular kernel classifiers (a set of classifiers containing those that achieve optimality). Our results highlight the benefit of using deep networks for classification tasks, in contrast to regression tasks, where excessive depth is harmful.

==> Old_Files/old_latex.tex <==
\begin{theorem}
\label{thm: Consistency conditions for classification}
    Let $\mathbb{P}_{(x, y)}$ denote the joint distribution over samples $x \in \mathcal{S}_+^{d-1}$ with $d \geq 2$ and labels $y \in \{-1, 1\}$ such that $\mathbb{P}(x | y = \ell)$ is Riemann integrable for $\ell \in \{-1, 1\}$.  Let $\mathbb{P}(y = 1) = p$ and let $m(x) = \arg \max_{\ell \in \{-1, 1\}} \mathbb{P}(y = \ell | x)$ denote the Bayes optimal classifier.  Let $\{\psi_L(\xi): [0, 1] \to \mathbb{R}_+\}_{L \in \mathbb{Z}_+}$ be bounded, monotonically increasing, continuous functions such that $\psi_L(\xi) \geq \frac{\xi^{\alpha}}{(1 - \xi^{\beta} + h(L))^{\frac{d-1}{2}}}$ with $h(L), \alpha \geq 0$, $\beta \geq 1$ and $\lim\limits_{L \to \infty} h(L) = 0$ and $\lim\limits_{L \to \infty} \psi_L(1) = \infty$.  Let $m_{n, L} (x) =  \sign\left(\frac{1}{n} \sum_{i=1}^{n} y^{(i)} \psi_L(x^T x^{(i)}) \right)$. Then for almost all $x \in \mathcal{S}_+^{d-1}$, $\lim\limits_{L \to \infty} \lim\limits_{n \to \infty} m_{n, L}(x) = m(x)$, in probability.
\end{theorem}


\begin{proof}
Let $\{x\} \cup \{x^{(i)}\}_{i=1}^{n} \in \mathcal{S}_+^{d-1}$.  Let $m_{n, L}(x) = \sign\left(\frac{1}{n} \sum_{i=1}^{n} y^{(i)} \psi_L(x^T x^{(i)}) \right)$ denote the classifier.  Now as $n \to \infty$, we can use the law of large numbers to simplify the integrand.  In particular, we have in probability: 
\begin{align*}
    \lim_{n \to \infty} m_{n, L} (x) &= \sign \left( \mathbb{E}_{(\tilde{x}, \tilde{y})} \left[ \tilde{y} \psi_L(x^T \tilde{x})  \right] \right) \\
    &= \sign \left( \sum_{\ell \in \{-1, 1\}}  \int_{\mathcal{S}_+^{d-1}}  \tilde{y} \mathbb{P}(\tilde{y} = \ell) \mathbb{P}(x^T \tilde{x}| \tilde{y} = \ell)  \psi_L(x^T \tilde{x}) d \tilde{x} \right) \\
    &= \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{\mathcal{S}_+^{d-1}} \mathbb{P}(x^T \tilde{x} | \tilde{y} = \ell)  \psi_L(x^T\tilde{x})) d \tilde{x} \right)
\end{align*}
To simplify integration over the intersection between the non-negative orthant and the sphere, we parameterize $x, x^{(i)}$ in terms of hyper-spherical angles $(\phi_1, \phi_2, \ldots, \phi_{d-1}) \in \left[0, \frac{\pi}{2} \right]^{d-1}$ and utilize rectangular partitions along these angles to approximate the densities $\mathbb{P}(\tilde{x} | \tilde{y} = \ell)$ for $\ell \in \{-1, 1\}$.  To ease notation, we write $\tilde{x} \in R$ to denote that the spherical angles of $\tilde{x}$ lie in the rectangle $R \subset \left[0, \frac{\pi}{2}\right]^{d-1}$.

Let $f_{\ell}(\tilde{x}) = \mathbb{P}(\tilde{x} | \tilde{y} = \ell)$.  As $f_1, f_{-1}$ are Riemann integrable, for any $\epsilon > 0$, select $k$ such that there exists a partition of $\left[0, \frac{\pi}{2}\right]^{d-1}$ given by rectangles $\{R_i = [\beta_{i-1}^{(1)}, \beta_i^{(1)}] \times \ldots \times [\beta_{i-1}^{(d-1)}, \beta_i^{(d-1)}]\}_{i=1}^{k}$ and non-negative $h_{\ell}(\tilde{x})$ with $\sup_{\tilde{x} \in \mathcal{S}_+^{d-1}} |h_{\ell}| < \epsilon$ for $\ell \in \{-1, 1\}$ satisfying: 
\begin{align*}
    f_1(\tilde{x}) &= h_1(\tilde{x}) + \sum_{i=1}^{k} \alpha_{i, 1} \chi_{\tilde{x} \in R_i} \\
    f_{-1}(\tilde{x}) &= h_{-1}(\tilde{x}) + \sum_{i=1}^{k} \alpha_{i, -1} \chi_{\tilde{x} \in R_i} \\
\end{align*}
Hence, by utilizing the approximation for $f_1, f_{-1}$ given by the rectangular partition, we have: 
\begin{align*}
     \lim_{n \to \infty} m_{n, L} (x) &=  \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{\mathcal{S}_+^{d-1}} \mathbb{P}(x^T \tilde{x} | \tilde{y} = \ell)  \psi_L(x^T\tilde{x})) d \tilde{x} \right) \\
     &= \sign \left( \sum_{i=1}^{k} \left[ p \alpha_{i, 1} - (1-p)  \alpha_{i, -1} + O(\epsilon) \right] \int_{R_i}  \psi_L(x^T\tilde{x})) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} \right)
\end{align*}

To further simplify the form above, we define: 
\begin{align*}
    k_{i, L}(x) := \int_{R_i}   \psi_L(x^T\tilde{x})) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} ~~;
\end{align*}
and hence, we have: 
\begin{align*}
    \lim_{n \to \infty} m_{n, L} (x)      &= \sign \left( \sum_{i=1}^{k} \left[ p \alpha_{i, 1} - (1-p)  \alpha_{i, -1} + O(\epsilon) \right] k_{i, L}(x) \right)
\end{align*}

Now we observe that $\sign(p \alpha_{i, 1} - (1-p) \alpha_{i, -1})$ is $O(\epsilon)$ from the prediction of the Bayes optimal classifier for any $x \in R_i$.  In particular, for $x \in R_i$: 
\begin{align*}
    m(x) &= \sign\left( pf_1(x) - (1-p) f_{-1}(x)\right) \\
    &= \sign\left(\left(p \left(h_1(x) + \sum_{j=1}^{k} \alpha_{j, 1} \chi_{x \in R_j} \right)  - (1-p)\left(h_{-1}(x) + \sum_{j=1}^{k} \alpha_{j, -1} \chi_{x \in R_j} \right)\right) \right) \\
    &= \sign\left( p h_1(\tilde{\theta}) - (1-p) h_{-1}(x)  + p \alpha_{i, 1} - (1-p) \alpha_{i, -1} \right) \\
    &= \sign\left( O(\epsilon)  + p \alpha_{i, 1} - (1-p) \alpha_{i, -1} \right)
\end{align*}

Hence, if $x \in R_i$ and $k_{i, L}(x) \to \infty$ as $L \to \infty$ while $k_{j, L}(x)$ is bounded for all $j \neq i$, we conclude that the prediction from $m_n(x)$ matches that of the Bayes optimal classifier.  Hence, the problem reduces to determining the conditions on $\psi$ under which the integral in $k_{i, L}(x)$ diverges for $x \in R_i$.  

We now show $k_{i, L}(x)$ diverges given the assumption on the $\psi_L$ in the theorem.  We will first need to present a lower bound on the integral by writing $x, x^{(i)}$ in terms of hyper-spherical angles.  In particular, we have
\begin{align*}
    x &= (\cos(\phi_1), \sin(\phi_1) \cos(\phi_2),  \ldots, \sin(\phi_1) \cdot \ldots \cdot \cos(\phi_{d-1}), \sin(\phi_1) \cdot \ldots \cdot \sin(\phi_{d-1})) \\
    x^{(i)} &= (\cos(\phi_1^{(i)}), \sin(\phi_1^{(i)}) \cos(\phi_2^{(i)}), \ldots, \sin(\phi_1^{(i)}) \cdot \ldots \cdot \cos(\phi_{d-1}^{(i)}), \sin(\phi_1^{(i)}) \cdot \ldots \cdot \sin(\phi_{d-1}^{(i)}))
\end{align*}
Given the forms above, we will use induction on the dimension $d$ to establish show that for $d \geq 2$: 
\begin{align*}
    x^T x^{(i)} &\geq \prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)})
\end{align*}
Naturally, the statement holds for $d = 2$, since we have $x^T x^{(i)} = \cos(\phi_1) \cos(\phi_1^{(i)} + \sin(\phi_1) \sin(\phi_1^{(i)})= \cos(\phi_1 - \phi_1^{(i)})$.  Now we assume for the sake of induction that the statement holds for $d = k-1$.  Then for $d = k - 1$, we have: 
\begin{align*}
    x^T x^{(i)} = \cos(\phi_1) \cos(\phi_1^{(i)}) + \sin(\phi_1) \sin(\phi_1^{(i)}) (z^T z^{(i)}) ~;
\end{align*}
where $z, z^{(i)} \in \mathcal{S}_+^{d-2}$ with hyper-spherical angles $(\phi_2, \phi_3, \ldots, \phi_{d-1})$ and $(\phi_2^{(i)}, \phi_3^{(i)}, \ldots, \phi_{d-1}^{(i)})$ respectively. Hence, we conclude by the inductive hypothesis: 
\begin{align*}
    x^T x^{(i)} &= \cos(\phi_1) \cos(\phi_1^{(i)}) + \sin(\phi_1) \sin(\phi_1^{(i)}) z^T z^{(i)} \\
    &\geq  \cos(\phi_1) \cos(\phi_1^{(i)}) + \sin(\phi_1) \sin(\phi_1^{(i)}) \prod_{j=2}^{d-1} \cos(\phi_j - \phi_j^{(i)}) \\
    &= \prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)}) + \cos(\phi_1) \cos(\phi_1^{(i)})\left( 1  - \prod_{j=2}^{d-1} \cos(\phi_j - \phi_j^{(i)}) \right) \\
    &\geq \prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)}) ; 
\end{align*}
where the last inequality follows from the fact that $\phi_1, \phi_1^{(i)} \in \left[0, \frac{\pi}{2}\right]$.  

Now suppose $x \in R_i$, then we utilize the lower bound on $x^T x^{(i)}$ and the fact that $psi_L$ are monotonically increasing to conclude: 
\begin{align*}
    k_{i, L}(x) &= \int_{R_i} \psi_L(x^T\tilde{x})) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} \geq \int_{R_i} \psi\left(\prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)})\right) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} 
\end{align*}

Now, as $x \in R_i$, we select $\epsilon > 0$ and restrict the domain of integration to those regions where each $\tilde{\phi_{j}} \in [\phi_{j} - \epsilon, \phi_j]$ such that $\cos(\phi_j - \tilde{\phi_j})$ is monotonically increasing.  We can always do so provided that $\phi_{j} \neq 0$, which is only violated on a measure zero set.  Then, we have: 
\begin{align*}
    k_{i, L}(x) &\geq \int_{\phi_1 - \epsilon}^{\phi_1} \ldots \int_{\phi_{d-1} - \epsilon}^{\phi_{d-1}} \psi\left(\prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)})\right) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} \\
    &= \int_{\cos(\epsilon)}^{1} \ldots \int_{\cos(\epsilon)}^{1} \psi\left(\prod_{j=1}^{d-1} u_j \right) \prod_{j=1}^{d-1} \frac{1}{\sqrt{1 - u_j^2}} d u_{d-1} \ldots d u_1 \\
    &\geq \int_{\cos(\epsilon)}^{1} \int_{u_1}^{1} \ldots \int_{u_1}^{1} \psi\left(\prod_{j=1}^{d-1} u_j \right) \prod_{j=1}^{d-1} \frac{1}{\sqrt{1 - u_j^2}} d u_{d-1} \ldots d u_2 d u_1 \\
    &\geq \int_{\cos(\epsilon)}^{1} \psi\left( u_1^{d-1} \right) \frac{(1- u_1)^{d-2}}{(1 - u_1^2)^{\frac{d-1}{2}}} d u_1
\end{align*}
Now, we utilize the assumption on $\psi$ given the theorem to conclude: 
\begin{align*}
    k_{i, L}(x) &\geq \int_{\cos(\epsilon)}^{1} \psi\left( u_1^{d-1} \right) \frac{(1- u_1)^{d-2}}{(1 - u_1^2)^{\frac{d-1}{2}}} d u_1 \\
    &\geq \int_{\cos(\epsilon)}^{1} \frac{u_1^{\alpha(d-1)}}{(1 -  u_1^{\beta(d-1)} + h(L))^{\frac{d-1}{2}}} \frac{(1- u_1)^{d-2}}{(1 - u_1^2)^{\frac{d-1}{2}}} d u_1 \\ 
    &\geq \frac{\cos(\epsilon)^{\alpha(d-1)}}{2^{\frac{d-1}{2}}} \int_{\cos(\epsilon)}^{1} \left(\frac{1- u_1}{1 -  u_1^{\beta(d-1)} + h(L)}\right)^{\frac{d-1}{2}} \frac{1}{(1 - u_1)} d u_1 \\
    &\geq \frac{\cos(\epsilon)^{\alpha(d-1)}}{(2\beta(d-1))^{\frac{d-1}{2}} } \int_{\cos(\epsilon)}^{1} \left(\frac{1- u_1}{1 -  u_1 + \frac{h(L)}{d-1}}\right)^{\frac{d-1}{2}} \frac{1}{(1 - u_1)} d u_1 \\
    &\geq \frac{\cos(\epsilon)^{\alpha(d-1)}}{(2\beta(d-1))^{\frac{d-1}{2}} } \int_{\cos(\epsilon)}^{1} \frac{(1- u_1)^{\frac{d-1}{2}}}{(1 -  u_1 + \frac{h(L)}{d-1})^{\frac{d+1}{2}}}   d u_1 \\
    &= -\frac{\cos(\epsilon)^{\alpha(d-1)}}{(2\beta(d-1))^{\frac{d-1}{2}} }  \int_{1-\cos(\epsilon)}^{0} \frac{v^{\frac{d-1}{2}}}{\left(v + \frac{h(L)}{d-1}\right)^{\frac{d+1}{2}}}  d v \\
    &= \frac{\cos(\epsilon)^{\alpha(d-1)}}{(2\beta(d-1))^{\frac{d-1}{2}} } \left( -\ln\left| \frac{h(L)}{d-1} \right| + \theta(1) \right) ~;
\end{align*}
where the last line follows from using a partial fraction decomposition to compute the integral.  Now as $h(L)$ approaches $0$, we conclude the corresponding integral diverges since $\lim\limits_{L \to 0} -\ln\left| \frac{h(L)}{d-1} \right| = \infty$.  

\end{proof}
%     &\geq \frac{1}{2^{\frac{d-1}{2}}(d-1 + h(L))^{\frac{d-1}{2}}} \int_{\cos(\epsilon)}^{1}  \frac{(1- u_1)^{d-2}}{(1 - u_1 + h(L))^{d-1}} d u_1


% Let $x = (\cos \theta, \sin \theta)$ and $x^{(i)} = (\cos \theta_i, \sin \theta_i)$, then the classifier simplifies to: 
% \begin{align*}
%     m_{n, L}(\theta) = \sign \left( \frac{1}{n} \sum_{i=1}^{n} y^{(i)} \psi_L(\cos(\theta - \theta_i)) \right)
% \end{align*}
% Now as $n \to \infty$, we can use the law of large numbers to simplify the integrand.  In particular, we have: 
% \begin{align*}
%     \lim_{n \to \infty} m_{n, L} (\theta) &= \sign \left( \mathbb{E}_{(\tilde{\theta}, \tilde{y})} \left[ \tilde{y} \psi_L(\cos(\theta - \tilde{\theta}))  \right] \right) \\
%     &= \sign \left( \sum_{\ell \in \{-1, 1\}}  \int_{0}^{\frac{\pi}{2}}  \tilde{y} \mathbb{P}(\tilde{y} = \ell) \mathbb{P}(\tilde{\theta} | \tilde{y} = \ell)  \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} \right) \\
%     &= \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{0}^{\frac{\pi}{2}} \mathbb{P}(\tilde{\theta} | \tilde{y} = \ell)  \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} \right)
% \end{align*}
% Let $f_{\ell}(\tilde{\theta}) = \mathbb{P}(\tilde{\theta} | \tilde{y} = \ell)$.  As $f_1, f_{-1}$ are Riemann integrable, for any $\epsilon > 0$, select $k$ such that there exists a partition of $[0, \frac{\pi}{2}]$ given by $I_i = [\beta_{i-1}, \beta_i]$ and non-negative $h_{\ell}(\tilde{\theta})$ with $\sup_{\tilde{\theta} \in \left[0, \frac{\pi}{2}\right]} |h_{\ell}| < \epsilon$ for $\ell \in \{-1, 1\}$ satisfying: 
% \begin{align*}
%     f_1(\tilde{\theta}) &= h_1(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, 1} \chi_{[\beta_{i-1}, \beta_{i}]} \\
%     f_{-1}(\tilde{\theta}) &= h_{-1}(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, -1} \chi_{[\beta_{i-1}, \beta_{i}]} \\    
% \end{align*}
% % We consider the case where $ $ is  Riemann integrable, and we take a sufficiently fine partition of the desired interval for both functions given by $\ell = 1$ and $\ell = -1$.  We consider the simple case where the characteristic functions are the same for both $\mathbb{P}(\tilde{\theta} | \tilde{y} = 1)$ and $\mathbb{P}(\tilde{\theta} | \tilde{y} = -1)$.  Namely, let $\{[\beta_{i-1}, \beta_{i}]\}_{i=1}^{k}$ denote a partition of $[0, \frac{\pi}{2}]$ and let 
% % \begin{align*}
% %     \mathbb{P}(\tilde{\theta} | \tilde{y} = 1) &= \sum_{i=1}^{k} \alpha_{i, 1} \chi_{[\beta_{i-1}, \beta_{i}]} \\
% %     \mathbb{P}(\tilde{\theta} | \tilde{y} = -1) &= \sum_{i=1}^{k} \alpha_{i, -1} \chi_{[\beta_{i-1}, \beta_{i}]}    
% % \end{align*}

% Then, we have: 
% \begin{align*}
%      \lim_{n \to \infty} m_{n, L} (\theta) &= \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{0}^{\frac{\pi}{2}} f_{\ell}(\tilde{\theta})  \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} \right)  \\
%      &= \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{0}^{\frac{\pi}{2}}  \left[ h_{\ell}(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, \ell} \chi_{[\beta_{i-1}, \beta_{i}]} \right] \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} \right) \\
%      &= \sign \left( \sum_{i=1}^{k} \left(p \alpha_{i, 1} - (1-p) \alpha_{i, -1} + O(\epsilon)\right) \int_{\beta_{i-1}}^{\beta_{i}} \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta}  \right)
% \end{align*}
% Lastly, we define 
% $$k_{i, L}(\theta) :=  \int_{\beta_{i-1}}^{\beta_{i}} \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} ,$$
% and we note that the $k_{i, L}$ are non-negative since the integrand is necessarily non-negative, as the support is given by $x, x^{(i)} \in \mathcal{S}_+^1$. Thus, we conclude that in probability: 
% \begin{align*}
%      \lim_{n \to \infty} m_{n, L} (\theta) &= \sign \left( \sum_{i=1}^{k} (p \alpha_{i, 1} - (1-p) \alpha_{i, -1} + O(\epsilon)) k_{i, L}(\theta) \right)
% \end{align*}
% Now we observe that $\sign(p \alpha_{i, 1} - (1-p) \alpha_{i, -1})$ is $O(\epsilon)$ from the prediction of the Bayes optimal classifier for any $\theta \in [\beta_{i-1}, \beta_i]$.  In particular, given $x = (\cos\theta, \sin\theta)$ with $\theta \in [\beta_{i-1}, \beta_i]$: 
% \begin{align*}
%     m(x) &= \sign\left( pf_1(\theta) - (1-p) f_{-1}(\theta)\right) \\
%     &= \sign\left(\left(p \left(h_1(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, 1} \chi_{[\beta_{i-1}, \beta_{i}]}(\theta) \right)  - (1-p)\left(h_{-1}(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, -1} \chi_{[\beta_{i-1}, \beta_{i}]}(\theta) \right)\right) \right) \\
%     &= \sign\left( p h_1(\tilde{\theta}) - (1-p) h_{-1}(\tilde{\theta})  + p \alpha_{i, 1} - (1-p) \alpha_{i, -1} \right) \\
%     &= \sign\left( O(\epsilon)  + p \alpha_{i, 1} - (1-p) \alpha_{i, -1} \right)
% \end{align*}

% Hence, if as $L \to \infty$, the $k_{i, L}(\theta)$ are functions that diverge only on $[\beta_{i-1}, \beta_i]$, then predictions given by $m_{n, L}(\theta)$ will match the predictions of the Bayes optimal classifier in probability.  Suppose that $\beta_{i-1} > 0$ and $\theta \in [\beta_{i-1}, \beta_i]$. Then, we have:
% \begin{align*}
%     k_{i, L}(\theta) &=  \int_{\beta_{i-1}}^{\beta_{i}} \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta}  \\ 
%     &\geq \int_{\theta - \epsilon}^{\theta} \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} ~~ \text{for $\epsilon$ such that $\cos(\theta - \tilde{\theta})$ is monotonic.}\\
%     &= \int_{\cos(\epsilon)}^{1} \frac{\psi(u)}{\sqrt{1-u^2}} du \\ 
%     &= \int_{\cos(\epsilon)}^{1} \frac{u}{\sqrt{1 - u^2 + h(L)}\sqrt{1-u^2}} \\
%     &\geq \int_{\cos(\epsilon)}^{1} \frac{u}{1 - u^2 + h(L)} \\
%     &= -\frac{1}{2} \ln | 1 - u^2 + h(L)| \biggr\rvert_{\cos(\epsilon)}^{1}\\
%     &= - \frac{1}{2} \ln | h(L)| +  \frac{1}{2} \ln | \sin(\epsilon) + h(L)|
% \end{align*}
% As $\sin(\epsilon) > 0$, we conclude that $\lim_{L \to \infty} \left( - \frac{1}{2} \ln | h(L)| +  \frac{1}{2} \ln | \sin(\epsilon) + h(L)|\right) = \infty$.  Hence, we conclude that the $\lim_{L \to \infty} k_{i, L} = \infty$ if  $\theta \in [\beta_{i-1}, \beta_i]$.  The case for $\beta_i = 0$ follows from instead restricting to the interval $[\theta, \theta + \epsilon]$, and so, we conclude that $\lim_{L \to \infty} \lim_{n \to \infty} m_{n, L}(x) = m(x)$ in probability.  \textcolor{red}{Adit: Technically, we need to assume that the argument of the sign function is nonzero and then take $L$ large enough such that the $k_{i, L}$ term dominates and then conclude the result.}





\subsection*{Infinite Depth NNGP Kernels are Singular Kernel Smoothers}
\textcolor{red}{We first establish conditions on the dual activation under which the NNGP kernel approaches an averaging kernel with sufficiently large depth.}

\begin{theorem}
\label{thm: NNGP averaging kernel} 
Let $\Sigma^{(L)}: [-1, 1] \to \mathbb{R}$ denote the NNGP kernel of a depth $L$, fully connected network with normalized activation $\phi$.  Let $(X, y) \in \mathcal{S}^{d-1 \times n} \times \mathbb{R}^{d_o \times n}$ denote a set of $n$ linearly independent training examples and labels.  Suppose $\check{\phi}$ has a unique attractor at $0$.  Then for any $\epsilon > 0$, there exists $L_0$ such that for $L > L_0$, 
\begin{align*}
    \left|y \Sigma^{(L)}(X, x) - y {\Sigma^{(L)}}^{-1}\Sigma^{(L)}(X, x) \right| < \epsilon
\end{align*}
\end{theorem}

\begin{proof}
Since, $0$ is the unique attractor of $\check{\phi}$, we must have for any $\lim_{L \to \infty} \check{\phi}^{(L)}(\xi) = 0$ for $\xi \in \mathbb{R}$ such that $\check{\phi}(\xi) \neq \xi$.  Hence since $n$ is finite, for any $h > 0$, there exists an $L_0$ such that for $L > L_0$: 
\begin{align*}
    1 - h n^2 \leq \|\Sigma^{(L)}(X, X)\|_2 \leq 1 + h n^2
\end{align*}
Hence, we have: 
\begin{align*}
    \left| y \Sigma^{(L)}(X, x) - y {\Sigma^{(L)}}^{-1}\Sigma^{(L)}(X, x) \right| &\leq \left\|y \right\| \left\| \Sigma^{(L)}(X, x) \right\| \left\| I - {\Sigma^{(L)}}^{-1} \right\| \leq n \left( 1 - \frac{1}{1 + h n^2}\right) 
\end{align*}
Taking $h = \frac{n - \epsilon}{n}$ gives the result.  
% Taking $h = \left(\frac{1}{1 - \frac{\epsilon}{n}} - 1\right) \frac{1}{n^2}$ gives the desired result.  
\end{proof}

\textcolor{red}{We then provide examples of activation functions satisfying the above conditions.}



\textbf{Remarks.}  The conditions of Theorem \ref{thm: NNGP averaging kernel} are satisfied for $\phi(x) = \sqrt{\frac{2e}{e^2 - 1}} \sin(x) $ and for $\phi(x) = \sqrt{\frac{1}{\arcsin{2/3}}} \erf(x)$.  Note that this condition is not true for ReLU or LeakyReLU and this gives rise to a significantly different infinite depth limit.  


\textcolor{red}{We then show that the infinite depth limit of such kernels has the following singularity property.}

\begin{prop}
\label{prop: Convergence of NNGP Ratio}
Let $\Sigma^{(L)}(\xi)$ denote the NNGP kernel of a depth $L$ network with normalized activation $\phi$. Suppose there exist $A, B\in \mathbb{R}$ with $B < 1$ such that $B\xi \leq \check{\phi}(\xi) \leq B(\xi + A\xi^2)$ for $\xi \in [0, 1]$.  Then, for any $\xi \in (0, 1)$ and any fixed $\epsilon \in (0,1)$, there exists $\psi: (0, 1) \to \mathbb{R}_+$ with $\lim_{\xi \to 1} \psi(\xi) = \infty$ such that:
\begin{align*}
    \frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)} < \frac{\xi}{\epsilon} \psi(\xi)
\end{align*}
\end{prop}
\begin{proof}
We have:
\begin{align*}
    \frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)} = \frac{\check{\phi} (\Sigma^{(L-1)}(\xi)) }{\check{\phi}(\Sigma^{(L-1)}(\epsilon))} \leq \frac{\Sigma^{(L-1)}(\xi) + A  (\Sigma^{(L-1)}(\xi))^2 }{\Sigma^{(L-1)}(\epsilon)} \leq \frac{\Sigma^{(L-1)}(\xi)}{\Sigma^{(L-1)}(\epsilon)} \left[ 1 + A \Sigma^{(L-1)}(\xi)\right]
\end{align*}
Therefore, starting with $\Sigma^{(0)}(\xi) = \xi$, we have: 
\begin{align*}
     \frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)} \leq \frac{\xi}{\epsilon} \prod_{i=0}^{L-1} \left[ 1 + A \Sigma^{(i)}(\xi)\right] \leq \frac{\xi}{\epsilon} \prod_{i=0}^{\infty} \left[ 1 + A \Sigma^{(i)}(\xi)\right]
\end{align*}
Now by \cite[Ch. 5, Proposition 3.1]{SteinComplexAnalysis}, the product on the right hand side converges iff $\sum_{i=0}^{\infty}|A \Sigma^{(i)}\xi|$ converges.  By the ratio test, we have: 
\begin{align*}
    \lim_{i \to \infty} \left|\frac{\Sigma^{(i)}(\xi)}{\Sigma^{(i-1)}(\xi)} \right| = \lim_{\xi \to 0} \frac{\check{\phi}(\xi)}{\xi} \leq \lim_{\xi \to 0} \frac{B (\xi + A \xi^2)}{\xi} = B < 1
\end{align*}
Hence, the series converges and so the product converges to a value, which we denote $\psi(\xi)$.  For $\xi = 1$, we have $\Sigma^{(L)}(\xi) = 1$ and so for any $\epsilon < 1$, $\lim_{L \to \infty}  \frac{\Sigma^{(L)}(1)}{\Sigma^{(L)}(\epsilon)} = \infty$.  Hence, we conclude that $\lim_{\xi \to 1} \psi(\xi) = \infty$.  
\end{proof}

\textcolor{red}{Again all the properties above hold for sine and erf activation functions.}

\begin{example}
If $\phi(x) = \sqrt{C}\sin(x) $ for $C = \frac{2e}{e^2 - 1} < 1$, then $\check{\phi}(\xi) = C \sinh(\xi)$.  Hence, $C\xi \leq \check{\phi}(\xi) \leq C(\xi + 2\xi^2)$. 
\end{example}

\begin{example}
If $\phi(x) = \sqrt{C} \erf(x)$ for $C = \frac{1}{\arcsin(\frac{2}{3})}$, then $\check{\phi}(\xi) = C \arcsin(\frac{2\xi}{3})$.  Hence, $\frac{2}{3}C x < \check{\phi}(\xi) \leq \frac{2}{3}C (\xi + 2 \xi^2)$.  
\end{example}

\textcolor{red}{We next show that the NNGP kernel converges exponentially in the depth to a smoothing kernel estimator.}

\begin{theorem}
\label{thm: exponential convergence of NNGP}
Let $\Sigma^{(L)}(\xi)$ denote the NNGP kernel of a depth $L$ network with normalized activation $\phi$. Suppose $\check{\phi}$ has a unique attractor at $0$ and that $\check{\phi}(\xi) = C g(A \xi)$ for constants $C, A \in \mathbb{R}$ satisfying $CA < 1$ and $A \leq 1$.  Lastly, suppose $\check{\phi}(\xi) \geq C A \xi$. Then, for $\xi \in (0, 1)$,
\begin{align*}
    C^L (g'(0)A)^{L-1} g(A \xi) \leq \Sigma^{(L)}(\xi) = (CA)^{L} \xi \psi_L(\xi) ~;
\end{align*}
for analytic $\psi_L(\xi): (0, 1) \to \mathbb{R}$ that are pointwise bounded by $\psi(\xi)$ for $\psi: (0,1) \to \mathbb{R}$ with $\lim_{\xi \to 1} \psi(\xi) = \infty$.  
\end{theorem}

\begin{proof}
We begin with the upper bound.  Let $M[f]$ denote the Carleman matrix for the function $f$, i.e. for $j, k \in \mathbb{N}$, $M[f]_{j,k} = \frac{1}{k!}\left[\frac{d^k (f(x)^j)}{dx^k} \right]\vert_{x = 0}$.  \textcolor{red}{(TODO Citation)} $M[f]$ has the following properties: 
\begin{enumerate}
    \item $M[f^{(L)}] = M[f]^L$, where $f^{(L)}(x) = f(f\ldots f(x))$ denotes composition by $f$ $L$ times.
    \item $\langle M[f^{(L)}]_{1, :}^T , [1, \xi, \xi^2, \ldots ]^T \rangle = f^{(L)}(\xi)$.  
\end{enumerate} 
In particular, when $f(x) = \sum_{n=1}^{\infty} a_n x^n$, $M[f]$ is an upper triangular matrix and so $M[f^{(L)}]$ is upper triangular for all $L$.  Note that $\check{\phi}(0) = 0$ by the attractor condition and so necessarily $M[\check{\phi}]$ is upper triangular.  The NNGP kernel at depth $L$ is given by the inner product between the first row of $M[\check{\phi}^{(L)}]$, which we denote $M[\check{\phi}^{(L)}]_{1, :}$, and $Z = [1, \xi, \xi^2, \ldots]$.  Since $M[f^{(L)}] = M[f]^L$, and since $M[f^{(L)}]$ is upper triangular, we have: 
\begin{align*}
    M[\check{\phi}^{(L)}]_{1,k} &= \sum_{i=1}^{k} M[\check{\phi}^{(L-1)}]_{1,i} M[\check{\phi}]_{i,k} \\
    &= \sum_{i=1}^{k} M[\check{\phi}^{(L-1)}]_{1,i} C A \gamma_{i,k}\\
    &= CA \sum_{i=1}^{k} M[\check{\phi}^{(L-1)}]_{1,i} \gamma_{i,k} ~;
\end{align*}
for some $\gamma_{i,k} \in \mathbb{R}$. Hence by induction, we have $M[\check{\phi}^{(L)}]_{1,k} = C^L A^L \beta_{k}(L)$ for some $\beta_k(L)$, which is a function of $L$. Therefore, we conclude: 
\begin{align*}
\Sigma^{(L)}(\xi) &= \langle M[\check{\phi}^{(L)}]_{1, :}^T , [1, \xi, \xi^2, \ldots ]^T \rangle \\
&= C^L A^L \sum_{i=1}^{\infty} \beta_i(L) \xi^{i} \\
&= C^L A^L \xi \sum_{i=0}^{\infty} \beta_{i+1}(L) \xi^{i}
\end{align*}
Hence, we have
\begin{align*}
    \frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)}  \leq \frac{\xi \sum_{i=0}^{\infty} \beta_{i+1}(L) \xi^{i}}{\epsilon } 
\end{align*}
Lastly, we know from Proposition \ref{prop: Convergence of NNGP Ratio} that $\frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)}$ converges.  Therefore, the coefficients $\beta_{i+1}(L)$ cannot diverge with $L$ and we conclude that:
$$ \Sigma^{(L)}(\xi) = (CA)^{L} \xi  \sum_{i=0}^{\infty} \beta_{i+1} \xi^{i} ~; $$
for $\{\beta_{j}\}_{j=1}^{\infty} \subset \mathbb{R}$ are independent of $\xi$.  Hence, we let $\psi_L(\xi) = \sum_{i=0}^{\infty} \beta_{i+1} \xi^{i}$, and since the $\beta_{i+1}$ do not diverge with $L$, we necessarily have that the functions are bounded above by some $\psi(\xi)$.  

Next, we prove the lower bound.  This again follows from an analysis of the terms of $M[\check{\phi}^{(L)}]_{1, :}$.  In particular, letting $[f]_k$ denote the $k^{th}$ coefficient of the Maclaurin series of $f$, we have 
$$M[\check{\phi}^{(L)}]_{1,k} \geq [\check{\phi}]_1^{L-1} [\check{\phi}]_k = (CAg'(0))^{L-1}  C \frac{d^k g}{dx^k}\left(0 \right) A^k . $$
Hence, by taking the inner product with the vector $[1, \xi, \xi^2, \ldots]$, we have that $\check{\phi}^{(L)}(\xi) \geq C^L (Ag'(0))^{L-1}) g(A \xi)$.  
\end{proof}

Again, the normalized activations for sine and erf satisfy the above conditions.  In particular, $C = \frac{2e}{e^2-1}, A = 1$ for the normalized sine activation and $C = \frac{1}{\arcsin(\frac{2}{3})}, A = \frac{2}{3}$ for the normalized $\erf$ activation.  Moreover, we have the following corollary.  

\begin{corollary}
For neural networks with normalized sine or erf activations and for $\xi \in (0, 1)$, the corresponding NNGP kernel of depth $L$ satisfies:
\begin{align}
    \Sigma^{(L)}(\xi) = (CA)^{L} \xi  \sum_{i=0}^{\infty} \beta_{2i+1} \xi^{2i} ~;
\end{align}
for constants $\{\beta_{2i+1}\}_{i=0}^{\infty}$ satisfying $\lim_{L \to \infty} \beta_{2i+1} < \infty$.  
\end{corollary}
\begin{proof}
The proof follows from a combinatorial argument. In particular, since the Taylor series expansions of the corresponding dual activations have no even powers, $M[\check{\phi}]_{jk}$ is nonzero iff the integer $k$ can be partitioned into $j$ blocks with only odd integers.  This is impossible when $j$ and $k$ have differing parity.  Hence, we conclude that $M[\check{\phi}]_{1, :} M[\check{\phi}]_{:, k} = 0$ whenever $k$ is even.  Hence, by induction, $M[\Sigma^{(L)}]_{1, k} = 0$ for all even $k$.  
\end{proof}

\textbf{Remarks.}  Empirically, for the normalized sine activation, we observe the stronger statement that the $\beta_{2i+1} \leq 1$ and in particular, we observe that $\Sigma^{(L)}(\xi) \leq (C)^{L} \frac{\xi}{1 - \xi^2}$ for $C = \frac{2e}{e^2-1}$.  As we show in the experiments section, this approximation is within 1\% of the performance of the deep NNGP for networks with the normalized sine activation.   

\subsection*{Infinite Depth NTKs are Singular Kernel Smoothers}
\textcolor{red}{We next establish conditions on the dual activation and its derivative such that the NTK kernel approaches a kernel smoother with sufficiently large depth. Note that the convergence is still exponential for the NTK. }

\begin{theorem}
\label{thm: NTK convergence to smoother}
Let $K^{L}: [-1, 1] \to \mathbb{R}$ denote the NTK of a depth $L$, fully connected network with normalized activation $\phi$.  Suppose that $\check{\phi}$ has a unique attractor at $0$ and that $\check{\phi}(\xi) = Cg(A\xi)$ for constants $C, A \in \mathbb{R}$ with $CA < 1$ and $A \leq 1$.  Suppose that $CA \leq \check{\phi}'(\xi) \leq CA(1 + B\xi^2)$ for $B \in \mathbb{R}$ for $\xi \in [0,1]$.  Let $(CA)^L \xi \leq \Sigma^{(L)}(\xi) \leq (CA)^L \xi \psi(\xi)$ as given by Theorem \ref{thm: exponential convergence of NNGP}.  Then for $\xi \in (0, 1)$, 
\begin{align*}
    (CA)^L \xi (1 + L) \leq K^{(L)}(\xi) <  (CA)^L e^{\frac{B\xi\psi(\xi)}{1 - CA}} \xi \left( 1 + \psi(\xi) L \right)  ~;
\end{align*}
and $\lim_{L \to \infty} K^{(L)}(1) = \infty$ if $\check{\phi}'(1) \geq 1$.  
\end{theorem}

\begin{proof}
The proof follows from that of Theorem \ref{thm: exponential convergence of NNGP} and the recursive formula for the NTK.  In particular, we have: 
\begin{align*}
    K^{(L)}(\xi) = K^{(L-1)}(\xi) \check{\phi}'(\Sigma^{(L-1)}(\xi)) + \Sigma^{(L)}(\xi) ~;~ K^{(0)}(\xi) = \xi
\end{align*} 
Unwinding the recursion, we have: 
\begin{align*}
    K^{(L)}(\xi) &= \xi \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] + \sum_{i=1}^{L} \left[ \Sigma^{(i)}(\xi) \prod_{j=i}^{L-1} \check{\phi}'(\Sigma^{(j)}(\xi))\right] \\
\end{align*}
    % &\leq \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] \left( \xi + \sum_{i=1}^{L} \Sigma^{(i)}(\xi) \right) ~~ \text{\textcolor{red}{TODO justification with convexity of dual}} \\
    % &\leq h(L) \left( \xi + \sum_{i=1}^{L} (CA)^i \xi \psi(\xi) \right) \\
    % &\leq h(L) \xi \left( 1 + \psi(\xi) \frac{1}{1 - CA}\right)
We now establish the upper bound.  Namely, using the assumption on $\Sigma^{(L)}(\xi)$ and the upper bound on $\check{\phi}'$, we have: 
\begin{align*}
    K^{(L)}(\xi) &= \xi \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] + \sum_{i=1}^{L} \left[ \Sigma^{(i)}(\xi) \prod_{j=i}^{L-1} \check{\phi}'(\Sigma^{(j)}(\xi))\right] \\
    &\leq \xi \left[\prod_{i=0}^{L-1} CA (1 + B (CA)^i \xi \psi(\xi)) \right] + \sum_{i=1}^{L} \left[ (CA)^i \xi \psi(\xi) \prod_{j=i}^{L-1} CA (1 + B (CA)^j \xi \psi(\xi))\right] \\
    &\leq \xi (CA)^L \left[\prod_{i=0}^{L-1}  e^{B (CA)^i \xi \psi(\xi)} \right] + \sum_{i=1}^{L} \left[ (CA)^i \xi \psi(\xi) (CA)^{L-i} \prod_{j=i}^{L-1}  e^{B (CA)^j \xi \psi(\xi)}\right] \\
    &\leq  \xi (CA)^L  e^{\frac{B \xi \psi(\xi)}{1-CA}}  + \sum_{i=1}^{L}  (CA)^L \xi \psi(\xi) e^{\frac{B \xi \psi(\xi)}{1-CA}} \\
    &\leq (CA)^L \xi e^{\frac{B \xi \psi(\xi)}{1-CA}} (1 + \psi(\xi)L )
\end{align*}

We similarly establish the lower bound.  
\begin{align*}
     K^{(L)}(\xi) &= \xi \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] + \sum_{i=1}^{L} \left[ \Sigma^{(i)}(\xi) \prod_{j=i}^{L-1} \check{\phi}'(\Sigma^{(j)}(\xi))\right] \\
     &\geq \xi \left[\prod_{i=0}^{L-1} CA \right] + \sum_{i=1}^{L} \left[ (CA)^i \xi \prod_{j=i}^{L-1} CA \right]\\
     &\geq \xi (CA)^L + \sum_{i=1}^{L} (CA)^L \xi \\
     &\geq \xi (CA)^L (1 + L)
\end{align*}

% The first inequality above follows from the fact that the dual activation is convex and non-decreasing on $[0, 1]$, and the fact that the derivative of a dual activation is itself a dual activation (without normalization by a constant factor).  Now, we analyze the convergence of the term $h(L) = \prod_{i=0}^{L} \check{\phi}'(\Sigma^{(i)}(\xi))$ as $L \to \infty$. The attractor condition on $\check{\phi}$ implies $\check{\phi}'(0) < 1$ and $\lim_{L \to \infty} \Sigma^{(L)}(\xi) = 0$.  Hence, there exists $L_0$ such that for $L > L_0$, $\check{\phi}'(\Sigma^{(L)}(\xi)) < 1$.  Therefore, $\lim_{L \to \infty} h(L) = 0$, which completes the proof of the upper bound.  
Lastly, we have that $K^{(L)}(1) = K^{(L-1)}(1) \check{\phi}'(1) + 1$, which must diverge (at least at rate $O(L)$) if $\check{\phi}'(1) \geq 1$.  
\end{proof}
\textcolor{red}{Naturally, the two activations we have considered throughout this work again satisfy all of the conditions of this theorem.   }

The following corollary connects the bound of the NNGP with that of the NTK.  In particular, as depth approaches infinity, the NTK has at most an extra exponential factor in $\xi \psi(\xi)$ on top of the bound of the NNGP. 
\begin{corollary}
Under the setting of Theorem \ref{thm: NTK convergence to smoother}, for any $\xi \in (0, 1)$ and any fixed $\epsilon \in (0,1)$: 
\begin{align*}
    \frac{\xi}{\epsilon} \frac{1}{\psi(\epsilon)} e^{-\frac{B \epsilon \psi(\epsilon)}{1-CA}}  \leq \lim_{L \to \infty} \frac{K^{(L)}(\xi)}{K^{(L)}(\epsilon)} \leq \frac{\xi}{\epsilon} \psi(\xi) e^{\frac{B \xi \psi(\xi)}{1-CA}} 
\end{align*}
\end{corollary}
% Under additional assumptions on the dual activation, the NTK also approaches a kernel smoother exponentially in the depth.  

% \begin{corollary}
%     Under the setting of Theorem \ref{thm: NTK convergence to smoother}, suppose that $\check{\phi}'(\xi) \leq CA(1 + B\xi^2)$ for $B \in \mathbb{R}$. Then, 
%     \begin{align*}
%             K^{(L)}(\xi) <  (CA)^L e^{\frac{B\xi}{1 - CA}} \xi \left( 1 + \psi(\xi) \frac{1}{1 - AC} \right)
%     \end{align*}
% \end{corollary}
% \begin{proof}
% Following the proof of Theorem \ref{thm: NTK convergence to smoother}, we have: 
% \begin{align*}
%     h(L) &=  \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] \\
%          &\leq \left[\prod_{i=0}^{L-1} \check{\phi}'(\xi (CA)^{i} \psi(\xi))\right] \\
%          &\leq \left[\prod_{i=0}^{L-1} CA (1 + B \xi (CA)^{i} \psi(\xi)) \right] \\
%          &\leq (CA)^L \left[\prod_{i=0}^{L-1}e^{B \xi (CA)^{i} \psi(\xi)} \right] \\
%          &\leq (CA)^L \exp\left(\sum_{i=0}^{\infty} B \xi (CA)^{i} \psi(\xi) \right) \\
%          &= (CA)^L \exp\left(\frac{B \xi\psi(\xi)}{1 - CA} \right)
% \end{align*}
% Hence, substituting into the result of Theorem \ref{thm: NTK convergence to smoother}, we conclude:
%     \begin{align*}
%             K^{(L)}(\xi) <  (CA)^L e^{\frac{B\xi}{1 - CA}} \xi \left( 1 + \psi(\xi) \frac{1}{1 - AC} \right)
%     \end{align*}
% \end{proof}


\subsection*{Infinite Depth ReLU NNGP Kernel and NTK}
\textcolor{blue}{Adit: Write out how the NNGP Kernel converges to the all 1's kernel and that the NTK for ReLU converges to a kernel that averages all class labels as the prediction.}



\section{Old Pole Order Analysis}
We now prove the result for the case where $\check{\phi}$ is replaced by a piece-wise linear function around $\xi = 0$ and $\xi = 1$.

\begin{lemma}
\label{lemma: piecewise linear NTK}
Let 
\begin{align*}
f(x) = \begin{cases} a x ~~ \text{if $x \in [0, c)$}  \\ g(x) ~~ \text{if $x \in [c, d)$} \\ 1 - b(1 - x) ~~ \text{if $x \in [d, 1]$}   \end{cases} ~~, ~~ h(x) = \begin{cases} a  ~~ \text{if $x \in [0, c]$}  \\ g'(x) ~~ \text{if $x \in (c, d)$} \\ b ~~ \text{if $x \in [d, 1]$}   \end{cases}  ~;
\end{align*}
such that $f(x)$ is strictly monotonically increasing and where $g(x)$ can be written as a convergent power series with non-negative coefficients and $0 < a < 1$ and $b > 1$.  For $L \geq 1 $, let 
$$k^{(L)}(x) = k^{(L-1)}(x) h(f^{(L-1)}(x)) + f^{(L)}(x)  ~~; ~~ k^{(0)}(x) = x. $$  
Then for $x \in (d, 1]$:
$$\lim_{L \to \infty} \frac{k^{(L)}(x)}{a^{L} (L + 1)} = \frac{R(x)}{(1 - x)^{-\log_b a}} ~~;$$
where $R(x)$ is bounded on $[0, 1]$.  
\end{lemma}
\begin{proof}
We consider the case of continuous $L$ (i.e. the flow instead of the discrete dynamical system).  In particular, as $0$ is the unique fixed point attractor of $f(x)$, we have for $x \in (d, 1)$ that after $L_0(x)$ time steps, $f^{(L_0(x))}(x) = f(d)$ and after $L_1$ time steps, $f^{(L_1)}(d) = f(c)$.   For any $L > L_0(x) + L_1$, we then have that $f^{(L)}(x) = a^{L - L_0(x) - L_1} f(c)$.  Hence there exists constant $x_0 > 0$ such that for $x \in (d, 1)$: 
\begin{align*}
    \lim_{L \to \infty}  \frac{a^{L - \lceil L_0(x) \rceil} f(x_0)}{a^L} \leq \lim_{L \to \infty} \frac{f^{(L)}(x)}{a^L} \leq \lim_{L \to \infty}  \frac{a^{L - L_0(x) - L_1} f(c)}{a^L} .
\end{align*}
Lastly, we can compute $L_0(x)$ by solving: 
\begin{align*}
    1 - b^{L_0(x)}(1 - x) = f(d) \implies L_0(x) = \log_a \left( \frac{1 - x}{1 - f(d)} \right)^{- \log_b a}
\end{align*}
Therefore, as $\lceil L_0(x) \rceil \geq L_0(x) - 1$, 
\begin{align*}
      \frac{af(x_0)}{ (1 - x)^{- \log_b a}} \leq \lim_{L \to \infty} \frac{f^{(L)}(x)}{a^L} \leq \frac{(1 - f(d))^{- \log_b a} f(c) }{a^{L_1} (1 - x)^{- \log_b a}} =  \frac{C}{ (1 - x)^{- \log_b a}} ~;
\end{align*}
for some positive constant $C$. Now via a similar analysis, we note that for $L > L_0(x) + L_1$, $h(f^{(L)}(x)) = a$.  Hence, for $L = L_0(x) + L_1 + T$ steps, we have by induction: 
\begin{align*}
    k^{(L)}(x) \leq a^{T} [k^{(L_0(x) + L_1)}(x) + T f(c)] = a^{L - L_0(x) - L_1} [k^{(L_0(x) + L_1)}(x) + (L - L_0(x) - L_1) f(c)]
\end{align*}
Now select $\tilde{C}(x)$ as a lower bound on the value of $k^{(L)}$ for $L$ such that $f^{(L)}(x) < c$.  Then, there exists some $x_0 \in [0, c)$ such that by induction on $L$: 
\begin{align*}
     k^{(L)}(x) \geq  a^{L - \lceil L_0(x) \rceil} [\tilde{C}(x) + (L - L_0(x) - L_1) f(x_0)]
\end{align*}
Therefore via the upper bound on $k^{(L)}(x)$: 
\begin{align*}
    \lim\limits_{L \to \infty} \frac{k^{(L)}(x)}{a^{L}(L+1)} &\leq \lim\limits_{L \to \infty} a^{-L_0(x) - L_1} \frac{k^{(L_0(x) + L_1)}(x) + (L - L_0(x) - L_1) f(c)}{L+1} \\
    &= a^{-L_0(x) - L_1} f(c) \\
    &= \frac{C}{ (1 - x)^{- \log_b a}} .
\end{align*}
Similarly, the lower bound on $k^{(L)}(x)$ yields: 
\begin{align*}
    \lim\limits_{L \to \infty} \frac{k^{(L)}(x)}{a^{L}(L+1)} & \geq  \frac{af(x_0)}{ (1 - x)^{- \log_b a}}, 
\end{align*}
which concludes the proof of the lemma. 
\end{proof}

Our first key observation is that Lemma \ref{lemma: piecewise linear NTK} can be extended to the case where $f$ is only linear around $0$. 

\begin{lemma}
\label{lemma: two piece pole order}
Let 
\begin{align*}
f(x) = \begin{cases} a x ~~ \text{if $x \in [0, c)$}  \\ g(x) ~~ \text{if $x \in [c, 1]$}  \end{cases} ~~, ~~ h(x) = \begin{cases} a  ~~ \text{if $x \in [0, c]$}  \\ g'(x) ~~ \text{if $x \in (c, 1]$} \end{cases} ~;
\end{align*}
such that $f(x)$ is monotonically increasing and where $g(x)$ can be written as a convergent power series with non-negative coefficients satisfying $g(1) = 1$ and $0 < a < 1$.  For $L \geq 1 $, let 
$$k^{(L)}(x) = k^{(L-1)}(x) h(f^{(L-1)}(x)) + f^{(L)}(x)  ~~; ~~ k^{(0)}(x) = x. $$  
Then for $x \in (d, 1]$:
$$\lim_{L \to \infty} \frac{k^{(L)}(x)}{a^{L} (L + 1)} = \frac{R(x)}{(1 - x)^{-\log_b a}} ~~;$$
where $R(x)$ is bounded in $[0, 1]$.  
\end{lemma}

\begin{proof}
We will first show that $\lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} = \frac{Q(x)}{(1 - x)^{-\log_b a}}$ for $Q(x)$ bounded in $[0, 1]$.  As $g(x)$ can be written as a convergent power series with non-negative coefficients with $g(1) = 1$, it is convex.  Hence, we upper bound $g(x)$ by the following function that is linear around $x = 0$ and $x = 1$: 
\begin{align*}
    f_{\epsilon}(x) = \begin{cases} a x ~~ \text{if $x \in [0, c)$}  \\ g(x) ~~ \text{if $x \in [c, 1-\epsilon)$} \\ 1 - (g'(1) - \epsilon)(1 - x) ~~ \text{if $x \in [1 - \epsilon, 1]$} \end{cases}
\end{align*}
Now by Lemma \ref{lemma: piecewise linear NTK} and as $f_{\epsilon}, f$ have the same normalizing factor $a$, we have that: 
\begin{align*}
    \lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} \leq \lim\limits_{L \to \infty} \frac{f_{\epsilon}^{(L)}(x)}{a^{L}} = \frac{Q_1(x)}{(1 - x)^{-\log_{g'(1) - \epsilon} a}}
\end{align*}
As $\epsilon$ is arbitrary, we conclude that the pole of $f$ at $x = 1$ has order at most $- \log_{g'(1)} a$.  Similarly, we can lower bound $f$ via the following function: 
\begin{align*}
    \tilde{f}(x) = \begin{cases} a x ~~ \text{if $x \in [0, d)$} \\ 1 - g'(1)(1 - x) ~~ \text{if $x \in [d, 1]$} \end{cases} ~;
\end{align*}
where $d$ is the intersection point of the tangent lines of $f$ at $x = 0$ and $x = 1$.  Again Lemma \ref{lemma: piecewise linear NTK} and as $\tilde{f}, f$ have the same normalizing factor $a$, we have that: 
\begin{align*}
 \lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} \geq \lim\limits_{L \to \infty} \frac{\tilde{f}^{(L)}(x)}{a^{L}} = \frac{Q_2(x)}{(1 - x)^{-\log_{g'(1)} a}}    
\end{align*}
Therefore, we conclude that: 
\begin{align*}
    \lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} = \frac{R(x)}{(1 - x)^{-\log_{g'(1)} a}} ~;
\end{align*}
for some $R(x)$ bounded in $[0, 1]$.  Now to bound the pole order of the normalized iteration of $k$ at $x =1$, we observe that there exists $L_0$ such that for $L \geq \lceil L_0 \rceil$, $f^{(L)}(x) \leq c$.  Hence, there exists some $x_0 \in [0, c)$ such that: 
\begin{align*}
    k^{(L)}(x) = a^{L - \lceil L_0 \rceil} (\tilde{C}(x) + (L - \lceil L_0 \rceil) f(x_0))
\end{align*}
Therefore, for $x \in (c, 1)$:
\begin{align*}
    \lim\limits_{L \to \infty} \frac{k^{(L)}(x)}{a^{L}(L+1)} = f(x_0) a^{ - \lceil L_0 \rceil} = \lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} =  \frac{R(x)}{(1 - x)^{-\log_{g'(1)} a}}, 
\end{align*}
which concludes the proof of the lemma.  
\end{proof}



We lastly need to establish a similar lower bound on the the above limit to conclude the proof.  We will construct the lower bound by first establishing the pole order of the NNGP iteration and then showing that the NNGP pole order is a lower bound on the NTK pole order.  Note that we have already established an upper bound on the pole order of the infinite depth NNGP via Eq.~\eqref{eq: NNGP approximation}.  Namely, by Eq.~\eqref{eq: NNGP approximation} and Lemma \ref{lemma: two piece pole order}: 
\begin{align*}
      \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} &= \lim_{\epsilon \to 0} \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi) - f_{\epsilon}^{(L)}(\xi)}{a^{L}} +  \lim_{\epsilon \to 0}  \lim\limits_{L \to \infty} \frac{f_{\epsilon}^{(L)}(\xi)}{a^{L}} \leq \frac{Q_1(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}} ~.
\end{align*}
Now, we alternatively lower bound $\check{\phi}$ via the following function: 
\begin{align*}
    \tilde{f}(\xi) = \begin{cases} a_1 \xi ~~ \text{if $x \in [0, c)$}  \\ 1 - \check{\phi}'(1)(1- \xi) ~~ \text{if $x \in [c, 1]$}  \end{cases} ~;
\end{align*}
where $\tilde{f}(c)$ corresponds to the intersection of the tangent lines of $\check{\phi}$ at $\xi = 0$ and $\xi = 1$.  As in the proof of Lemma \ref{lemma: two piece pole order}, we thus have that: 
\begin{align*}
    \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} \geq \lim\limits_{L \to \infty}  \frac{\tilde{f}^{(L)}(\xi)}{a^{L}} = \frac{Q_2(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}}
\end{align*}
Hence, we conclude that: 
\begin{align*}
    \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} = \frac{Q(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}} ~, 
\end{align*}
where we also know that $Q(\xi)$ can be written as a convergent power series on $[0, 1]$ with non-negative coefficients by definition of the NNGP iteration.  Lastly, we utilize Eq.~\ref{eq: Closed form for NTK} to show that: 
\begin{align*}
    \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} \leq  \lim\limits_{L \to \infty}  \frac{K^{(L)}(\xi)}{a^{L}(L+1)} ~.
\end{align*}
In particular, by Eq.~\ref{eq: Closed form for NTK}, we have: 
\begin{align*}
    K^{(L)}(\xi)= \sum_{i=0}^{L} \check{\phi}^{(i)}(\xi) \prod_{k=i}^{L-1} \check{\phi}'\left(\check{\phi}^{(k)}(\xi)\right) ~~;
\end{align*}
and we next write $\check{\phi}^{(i)}(\xi)$ as a product.  Namely, using the power series representation for $\check{\phi}$ and unrolling the iteration, we have: 
\begin{align*}
    \check{\phi}^{(i)}(\xi) &= \sum_{j=1}^{\infty} a_j \left(\check{\phi}^{(i-1)}(\xi)\right)^{j} \\
    &= a_1 \check{\phi}^{(i-1)}(\xi) \left (1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(i-1)}(\xi)\right)^{j} \right) \\
    &= a_1^{i} \xi \prod_{k=0}^{i - 1} \left( 1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j} \right) ~.
\end{align*}
We similar use the power series for $\check{\phi}'(\xi)$ to conclude: 
\begin{align*}
    \check{\phi}'\left(\check{\phi}^{(k)}(\xi)\right) &= \sum_{j=1}^{\infty} j a_j \left(\check{\phi}^{(k)}(\xi)\right)^{j-1} \\
    &\geq \sum_{j=1}^{\infty} a_j \left(\check{\phi}^{(k)}(\xi)\right)^{j-1} \\
    &\geq a_1 \left(1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j-1} \right) \\
    &\geq a_1 \left(1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j} \right) ~~ \left(\text{as $\check{\phi}^{(k)}(\xi) \leq 1$.} \right) ~. 
\end{align*}
Therefore, we simplify Eq.~\ref{eq: Closed form for NTK} as follows: 
\begin{align*}
      K^{(L)}(\xi) &= \sum_{i=0}^{L} \check{\phi}^{(i)}(\xi) \prod_{k=i}^{L-1} \check{\phi}'\left(\check{\phi}^{(k)}(\xi)\right) \\
      &\geq \sum_{i=0}^{L} a_1^{i} \xi \prod_{k=0}^{i - 1} \left( 1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j} \right) \prod_{k'=i}^{L-1} a_1 \left(1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k')}(\xi)\right)^{j} \right) \\
      &= \sum_{i=0}^{L} a_1^{i} \xi \prod_{k=0}^{L - 1} \left( 1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j} \right) \\
      &= (L+1) \check{\phi}^{(L)}(\xi) ~.
\end{align*}
Therefore, we conclude: 
\begin{align*}
    \frac{K^{(L)}(\xi)}{a^{L} (L + 1)} \geq \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} ~, 
\end{align*}
and so: 
\begin{align}
\label{eq: Lower bound on normalized iterated NTK}
    \lim\limits_{L \to \infty}  \frac{K^{(L)}(\xi)}{a^{L}(L+1)} \geq \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} = \frac{Q(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}}.
\end{align}
Lastly, we combine Eq.~\ref{eq: Lower bound on normalized iterated NTK} and \ref{eq: Upper bound on normalized iterated NTK} to conclude: 
\begin{align*}
   \frac{Q(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}} \leq \lim\limits_{L \to \infty}  \frac{K^{(L)}(\xi)}{a^{L}(L+1)} \leq \frac{\tilde{R}(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}}~. 
\end{align*}
Thus, by the squeeze theorem: 
\begin{align*}
    \lim\limits_{L \to \infty}  \frac{K^{(L)}(\xi)}{a^{L}(L+1)} = \frac{R(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}}~, 
\end{align*}
where $R(\xi)$ is bounded and by Eq.~\ref{eq: Closed form for NTK}, can be written as a power series with non-negative coefficients.  This concludes the proof of Theorem \ref{theorem: Dynamical Systems NTK}.    



We make use of the following lemma throughout our proofs. 

\begin{lemma}
\label{lemma: limit for order of pole}
Let $f(x): [0, 1] \to \mathbb{R}$ such that $f$ has a singularity only at $x = 1$. Then $x = 1$ is a singularity of order $\alpha$ iff for any $b > 1$:  
\begin{align}
\label{eq: log order of pole}
    -\log_b \left(\lim_{\epsilon \to 0^+}  \frac{f(1 - b\epsilon)}{f(1  - \epsilon)}\right) = \alpha.
\end{align}
\end{lemma}

\begin{proof}
Note that $f$ has a singularity of order $\alpha < \infty$ iff
\begin{align*}
    f(x) = \frac{R(x)}{(1 - x)^{\alpha}},
\end{align*}
where $R(x)$ is bounded on $[0, 1]$, $R(1) \neq 0$, and $R(x)$ is continuous at $1$.  Hence,  by directly substituting the closed form for $f$ into Eq.~\eqref{eq: log order of pole}, we have that: 
\begin{align*}
    -\log_b \left(\lim_{\epsilon \to 0^+}  \frac{f(1 - b\epsilon)}{f(1  - \epsilon)}\right) &= -\log_b \left(\lim_{\epsilon \to 0} \frac{R(1 - b\epsilon)}{R(1 - \epsilon)} b^{-\alpha} \right) = \alpha ~.
\end{align*}
If the pole has infinite order, then we necessarily have: 
\begin{align*}
    \lim_{\epsilon \to 0^+}  \frac{f(1 - b\epsilon)}{f(1  - \epsilon)} = 0 ~, 
\end{align*}
and so $\alpha = -\log_b(0) = \infty$.  The other direction follows by a similar line of reasoning.  In particular, suppose there exists $\alpha < \infty$ such that 
\begin{align*}
    -\log_b \left(\lim_{\epsilon \to 0^+}  \frac{f(1 - b\epsilon)}{f(1  - \epsilon)}\right) = \alpha.
\end{align*}
Then, as $f(x)$ has a singularity at $x = 1$, there exists $\beta < \infty$ such that
\begin{align*}
    f(x) = \frac{R(x)}{(1 - x)^{\beta}}~,
\end{align*}
where $R(x)$ is bounded on $[0, 1]$, $R(1) \neq 0$, and $R(x)$ is continuous at $1$.  We then conclude that $\beta = \alpha$.  
\end{proof}





















==> Optimality of Infinite Depth Neural Networks/Old_Files/old_latex.tex <==
\begin{theorem}
\label{thm: Consistency conditions for classification}
    Let $\mathbb{P}_{(x, y)}$ denote the joint distribution over samples $x \in \mathcal{S}_+^{d-1}$ with $d \geq 2$ and labels $y \in \{-1, 1\}$ such that $\mathbb{P}(x | y = \ell)$ is Riemann integrable for $\ell \in \{-1, 1\}$.  Let $\mathbb{P}(y = 1) = p$ and let $m(x) = \arg \max_{\ell \in \{-1, 1\}} \mathbb{P}(y = \ell | x)$ denote the Bayes optimal classifier.  Let $\{\psi_L(\xi): [0, 1] \to \mathbb{R}_+\}_{L \in \mathbb{Z}_+}$ be bounded, monotonically increasing, continuous functions such that $\psi_L(\xi) \geq \frac{\xi^{\alpha}}{(1 - \xi^{\beta} + h(L))^{\frac{d-1}{2}}}$ with $h(L), \alpha \geq 0$, $\beta \geq 1$ and $\lim\limits_{L \to \infty} h(L) = 0$ and $\lim\limits_{L \to \infty} \psi_L(1) = \infty$.  Let $m_{n, L} (x) =  \sign\left(\frac{1}{n} \sum_{i=1}^{n} y^{(i)} \psi_L(x^T x^{(i)}) \right)$. Then for almost all $x \in \mathcal{S}_+^{d-1}$, $\lim\limits_{L \to \infty} \lim\limits_{n \to \infty} m_{n, L}(x) = m(x)$, in probability.
\end{theorem}


\begin{proof}
Let $\{x\} \cup \{x^{(i)}\}_{i=1}^{n} \in \mathcal{S}_+^{d-1}$.  Let $m_{n, L}(x) = \sign\left(\frac{1}{n} \sum_{i=1}^{n} y^{(i)} \psi_L(x^T x^{(i)}) \right)$ denote the classifier.  Now as $n \to \infty$, we can use the law of large numbers to simplify the integrand.  In particular, we have in probability: 
\begin{align*}
    \lim_{n \to \infty} m_{n, L} (x) &= \sign \left( \mathbb{E}_{(\tilde{x}, \tilde{y})} \left[ \tilde{y} \psi_L(x^T \tilde{x})  \right] \right) \\
    &= \sign \left( \sum_{\ell \in \{-1, 1\}}  \int_{\mathcal{S}_+^{d-1}}  \tilde{y} \mathbb{P}(\tilde{y} = \ell) \mathbb{P}(x^T \tilde{x}| \tilde{y} = \ell)  \psi_L(x^T \tilde{x}) d \tilde{x} \right) \\
    &= \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{\mathcal{S}_+^{d-1}} \mathbb{P}(x^T \tilde{x} | \tilde{y} = \ell)  \psi_L(x^T\tilde{x})) d \tilde{x} \right)
\end{align*}
To simplify integration over the intersection between the non-negative orthant and the sphere, we parameterize $x, x^{(i)}$ in terms of hyper-spherical angles $(\phi_1, \phi_2, \ldots, \phi_{d-1}) \in \left[0, \frac{\pi}{2} \right]^{d-1}$ and utilize rectangular partitions along these angles to approximate the densities $\mathbb{P}(\tilde{x} | \tilde{y} = \ell)$ for $\ell \in \{-1, 1\}$.  To ease notation, we write $\tilde{x} \in R$ to denote that the spherical angles of $\tilde{x}$ lie in the rectangle $R \subset \left[0, \frac{\pi}{2}\right]^{d-1}$.

Let $f_{\ell}(\tilde{x}) = \mathbb{P}(\tilde{x} | \tilde{y} = \ell)$.  As $f_1, f_{-1}$ are Riemann integrable, for any $\epsilon > 0$, select $k$ such that there exists a partition of $\left[0, \frac{\pi}{2}\right]^{d-1}$ given by rectangles $\{R_i = [\beta_{i-1}^{(1)}, \beta_i^{(1)}] \times \ldots \times [\beta_{i-1}^{(d-1)}, \beta_i^{(d-1)}]\}_{i=1}^{k}$ and non-negative $h_{\ell}(\tilde{x})$ with $\sup_{\tilde{x} \in \mathcal{S}_+^{d-1}} |h_{\ell}| < \epsilon$ for $\ell \in \{-1, 1\}$ satisfying: 
\begin{align*}
    f_1(\tilde{x}) &= h_1(\tilde{x}) + \sum_{i=1}^{k} \alpha_{i, 1} \chi_{\tilde{x} \in R_i} \\
    f_{-1}(\tilde{x}) &= h_{-1}(\tilde{x}) + \sum_{i=1}^{k} \alpha_{i, -1} \chi_{\tilde{x} \in R_i} \\
\end{align*}
Hence, by utilizing the approximation for $f_1, f_{-1}$ given by the rectangular partition, we have: 
\begin{align*}
     \lim_{n \to \infty} m_{n, L} (x) &=  \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{\mathcal{S}_+^{d-1}} \mathbb{P}(x^T \tilde{x} | \tilde{y} = \ell)  \psi_L(x^T\tilde{x})) d \tilde{x} \right) \\
     &= \sign \left( \sum_{i=1}^{k} \left[ p \alpha_{i, 1} - (1-p)  \alpha_{i, -1} + O(\epsilon) \right] \int_{R_i}  \psi_L(x^T\tilde{x})) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} \right)
\end{align*}

To further simplify the form above, we define: 
\begin{align*}
    k_{i, L}(x) := \int_{R_i}   \psi_L(x^T\tilde{x})) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} ~~;
\end{align*}
and hence, we have: 
\begin{align*}
    \lim_{n \to \infty} m_{n, L} (x)      &= \sign \left( \sum_{i=1}^{k} \left[ p \alpha_{i, 1} - (1-p)  \alpha_{i, -1} + O(\epsilon) \right] k_{i, L}(x) \right)
\end{align*}

Now we observe that $\sign(p \alpha_{i, 1} - (1-p) \alpha_{i, -1})$ is $O(\epsilon)$ from the prediction of the Bayes optimal classifier for any $x \in R_i$.  In particular, for $x \in R_i$: 
\begin{align*}
    m(x) &= \sign\left( pf_1(x) - (1-p) f_{-1}(x)\right) \\
    &= \sign\left(\left(p \left(h_1(x) + \sum_{j=1}^{k} \alpha_{j, 1} \chi_{x \in R_j} \right)  - (1-p)\left(h_{-1}(x) + \sum_{j=1}^{k} \alpha_{j, -1} \chi_{x \in R_j} \right)\right) \right) \\
    &= \sign\left( p h_1(\tilde{\theta}) - (1-p) h_{-1}(x)  + p \alpha_{i, 1} - (1-p) \alpha_{i, -1} \right) \\
    &= \sign\left( O(\epsilon)  + p \alpha_{i, 1} - (1-p) \alpha_{i, -1} \right)
\end{align*}

Hence, if $x \in R_i$ and $k_{i, L}(x) \to \infty$ as $L \to \infty$ while $k_{j, L}(x)$ is bounded for all $j \neq i$, we conclude that the prediction from $m_n(x)$ matches that of the Bayes optimal classifier.  Hence, the problem reduces to determining the conditions on $\psi$ under which the integral in $k_{i, L}(x)$ diverges for $x \in R_i$.  

We now show $k_{i, L}(x)$ diverges given the assumption on the $\psi_L$ in the theorem.  We will first need to present a lower bound on the integral by writing $x, x^{(i)}$ in terms of hyper-spherical angles.  In particular, we have
\begin{align*}
    x &= (\cos(\phi_1), \sin(\phi_1) \cos(\phi_2),  \ldots, \sin(\phi_1) \cdot \ldots \cdot \cos(\phi_{d-1}), \sin(\phi_1) \cdot \ldots \cdot \sin(\phi_{d-1})) \\
    x^{(i)} &= (\cos(\phi_1^{(i)}), \sin(\phi_1^{(i)}) \cos(\phi_2^{(i)}), \ldots, \sin(\phi_1^{(i)}) \cdot \ldots \cdot \cos(\phi_{d-1}^{(i)}), \sin(\phi_1^{(i)}) \cdot \ldots \cdot \sin(\phi_{d-1}^{(i)}))
\end{align*}
Given the forms above, we will use induction on the dimension $d$ to establish show that for $d \geq 2$: 
\begin{align*}
    x^T x^{(i)} &\geq \prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)})
\end{align*}
Naturally, the statement holds for $d = 2$, since we have $x^T x^{(i)} = \cos(\phi_1) \cos(\phi_1^{(i)} + \sin(\phi_1) \sin(\phi_1^{(i)})= \cos(\phi_1 - \phi_1^{(i)})$.  Now we assume for the sake of induction that the statement holds for $d = k-1$.  Then for $d = k - 1$, we have: 
\begin{align*}
    x^T x^{(i)} = \cos(\phi_1) \cos(\phi_1^{(i)}) + \sin(\phi_1) \sin(\phi_1^{(i)}) (z^T z^{(i)}) ~;
\end{align*}
where $z, z^{(i)} \in \mathcal{S}_+^{d-2}$ with hyper-spherical angles $(\phi_2, \phi_3, \ldots, \phi_{d-1})$ and $(\phi_2^{(i)}, \phi_3^{(i)}, \ldots, \phi_{d-1}^{(i)})$ respectively. Hence, we conclude by the inductive hypothesis: 
\begin{align*}
    x^T x^{(i)} &= \cos(\phi_1) \cos(\phi_1^{(i)}) + \sin(\phi_1) \sin(\phi_1^{(i)}) z^T z^{(i)} \\
    &\geq  \cos(\phi_1) \cos(\phi_1^{(i)}) + \sin(\phi_1) \sin(\phi_1^{(i)}) \prod_{j=2}^{d-1} \cos(\phi_j - \phi_j^{(i)}) \\
    &= \prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)}) + \cos(\phi_1) \cos(\phi_1^{(i)})\left( 1  - \prod_{j=2}^{d-1} \cos(\phi_j - \phi_j^{(i)}) \right) \\
    &\geq \prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)}) ; 
\end{align*}
where the last inequality follows from the fact that $\phi_1, \phi_1^{(i)} \in \left[0, \frac{\pi}{2}\right]$.  

Now suppose $x \in R_i$, then we utilize the lower bound on $x^T x^{(i)}$ and the fact that $psi_L$ are monotonically increasing to conclude: 
\begin{align*}
    k_{i, L}(x) &= \int_{R_i} \psi_L(x^T\tilde{x})) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} \geq \int_{R_i} \psi\left(\prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)})\right) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} 
\end{align*}

Now, as $x \in R_i$, we select $\epsilon > 0$ and restrict the domain of integration to those regions where each $\tilde{\phi_{j}} \in [\phi_{j} - \epsilon, \phi_j]$ such that $\cos(\phi_j - \tilde{\phi_j})$ is monotonically increasing.  We can always do so provided that $\phi_{j} \neq 0$, which is only violated on a measure zero set.  Then, we have: 
\begin{align*}
    k_{i, L}(x) &\geq \int_{\phi_1 - \epsilon}^{\phi_1} \ldots \int_{\phi_{d-1} - \epsilon}^{\phi_{d-1}} \psi\left(\prod_{j=1}^{d-1} \cos(\phi_j - \phi_j^{(i)})\right) d \tilde{\phi_{d-1}} \ldots d \tilde{\phi_1} \\
    &= \int_{\cos(\epsilon)}^{1} \ldots \int_{\cos(\epsilon)}^{1} \psi\left(\prod_{j=1}^{d-1} u_j \right) \prod_{j=1}^{d-1} \frac{1}{\sqrt{1 - u_j^2}} d u_{d-1} \ldots d u_1 \\
    &\geq \int_{\cos(\epsilon)}^{1} \int_{u_1}^{1} \ldots \int_{u_1}^{1} \psi\left(\prod_{j=1}^{d-1} u_j \right) \prod_{j=1}^{d-1} \frac{1}{\sqrt{1 - u_j^2}} d u_{d-1} \ldots d u_2 d u_1 \\
    &\geq \int_{\cos(\epsilon)}^{1} \psi\left( u_1^{d-1} \right) \frac{(1- u_1)^{d-2}}{(1 - u_1^2)^{\frac{d-1}{2}}} d u_1
\end{align*}
Now, we utilize the assumption on $\psi$ given the theorem to conclude: 
\begin{align*}
    k_{i, L}(x) &\geq \int_{\cos(\epsilon)}^{1} \psi\left( u_1^{d-1} \right) \frac{(1- u_1)^{d-2}}{(1 - u_1^2)^{\frac{d-1}{2}}} d u_1 \\
    &\geq \int_{\cos(\epsilon)}^{1} \frac{u_1^{\alpha(d-1)}}{(1 -  u_1^{\beta(d-1)} + h(L))^{\frac{d-1}{2}}} \frac{(1- u_1)^{d-2}}{(1 - u_1^2)^{\frac{d-1}{2}}} d u_1 \\ 
    &\geq \frac{\cos(\epsilon)^{\alpha(d-1)}}{2^{\frac{d-1}{2}}} \int_{\cos(\epsilon)}^{1} \left(\frac{1- u_1}{1 -  u_1^{\beta(d-1)} + h(L)}\right)^{\frac{d-1}{2}} \frac{1}{(1 - u_1)} d u_1 \\
    &\geq \frac{\cos(\epsilon)^{\alpha(d-1)}}{(2\beta(d-1))^{\frac{d-1}{2}} } \int_{\cos(\epsilon)}^{1} \left(\frac{1- u_1}{1 -  u_1 + \frac{h(L)}{d-1}}\right)^{\frac{d-1}{2}} \frac{1}{(1 - u_1)} d u_1 \\
    &\geq \frac{\cos(\epsilon)^{\alpha(d-1)}}{(2\beta(d-1))^{\frac{d-1}{2}} } \int_{\cos(\epsilon)}^{1} \frac{(1- u_1)^{\frac{d-1}{2}}}{(1 -  u_1 + \frac{h(L)}{d-1})^{\frac{d+1}{2}}}   d u_1 \\
    &= -\frac{\cos(\epsilon)^{\alpha(d-1)}}{(2\beta(d-1))^{\frac{d-1}{2}} }  \int_{1-\cos(\epsilon)}^{0} \frac{v^{\frac{d-1}{2}}}{\left(v + \frac{h(L)}{d-1}\right)^{\frac{d+1}{2}}}  d v \\
    &= \frac{\cos(\epsilon)^{\alpha(d-1)}}{(2\beta(d-1))^{\frac{d-1}{2}} } \left( -\ln\left| \frac{h(L)}{d-1} \right| + \theta(1) \right) ~;
\end{align*}
where the last line follows from using a partial fraction decomposition to compute the integral.  Now as $h(L)$ approaches $0$, we conclude the corresponding integral diverges since $\lim\limits_{L \to 0} -\ln\left| \frac{h(L)}{d-1} \right| = \infty$.  

\end{proof}
%     &\geq \frac{1}{2^{\frac{d-1}{2}}(d-1 + h(L))^{\frac{d-1}{2}}} \int_{\cos(\epsilon)}^{1}  \frac{(1- u_1)^{d-2}}{(1 - u_1 + h(L))^{d-1}} d u_1


% Let $x = (\cos \theta, \sin \theta)$ and $x^{(i)} = (\cos \theta_i, \sin \theta_i)$, then the classifier simplifies to: 
% \begin{align*}
%     m_{n, L}(\theta) = \sign \left( \frac{1}{n} \sum_{i=1}^{n} y^{(i)} \psi_L(\cos(\theta - \theta_i)) \right)
% \end{align*}
% Now as $n \to \infty$, we can use the law of large numbers to simplify the integrand.  In particular, we have: 
% \begin{align*}
%     \lim_{n \to \infty} m_{n, L} (\theta) &= \sign \left( \mathbb{E}_{(\tilde{\theta}, \tilde{y})} \left[ \tilde{y} \psi_L(\cos(\theta - \tilde{\theta}))  \right] \right) \\
%     &= \sign \left( \sum_{\ell \in \{-1, 1\}}  \int_{0}^{\frac{\pi}{2}}  \tilde{y} \mathbb{P}(\tilde{y} = \ell) \mathbb{P}(\tilde{\theta} | \tilde{y} = \ell)  \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} \right) \\
%     &= \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{0}^{\frac{\pi}{2}} \mathbb{P}(\tilde{\theta} | \tilde{y} = \ell)  \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} \right)
% \end{align*}
% Let $f_{\ell}(\tilde{\theta}) = \mathbb{P}(\tilde{\theta} | \tilde{y} = \ell)$.  As $f_1, f_{-1}$ are Riemann integrable, for any $\epsilon > 0$, select $k$ such that there exists a partition of $[0, \frac{\pi}{2}]$ given by $I_i = [\beta_{i-1}, \beta_i]$ and non-negative $h_{\ell}(\tilde{\theta})$ with $\sup_{\tilde{\theta} \in \left[0, \frac{\pi}{2}\right]} |h_{\ell}| < \epsilon$ for $\ell \in \{-1, 1\}$ satisfying: 
% \begin{align*}
%     f_1(\tilde{\theta}) &= h_1(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, 1} \chi_{[\beta_{i-1}, \beta_{i}]} \\
%     f_{-1}(\tilde{\theta}) &= h_{-1}(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, -1} \chi_{[\beta_{i-1}, \beta_{i}]} \\    
% \end{align*}
% % We consider the case where $ $ is  Riemann integrable, and we take a sufficiently fine partition of the desired interval for both functions given by $\ell = 1$ and $\ell = -1$.  We consider the simple case where the characteristic functions are the same for both $\mathbb{P}(\tilde{\theta} | \tilde{y} = 1)$ and $\mathbb{P}(\tilde{\theta} | \tilde{y} = -1)$.  Namely, let $\{[\beta_{i-1}, \beta_{i}]\}_{i=1}^{k}$ denote a partition of $[0, \frac{\pi}{2}]$ and let 
% % \begin{align*}
% %     \mathbb{P}(\tilde{\theta} | \tilde{y} = 1) &= \sum_{i=1}^{k} \alpha_{i, 1} \chi_{[\beta_{i-1}, \beta_{i}]} \\
% %     \mathbb{P}(\tilde{\theta} | \tilde{y} = -1) &= \sum_{i=1}^{k} \alpha_{i, -1} \chi_{[\beta_{i-1}, \beta_{i}]}    
% % \end{align*}

% Then, we have: 
% \begin{align*}
%      \lim_{n \to \infty} m_{n, L} (\theta) &= \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{0}^{\frac{\pi}{2}} f_{\ell}(\tilde{\theta})  \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} \right)  \\
%      &= \sign \left( \sum_{\ell \in \{-1, 1\}} \tilde{y} \mathbb{P}(\tilde{y} = \ell)  \int_{0}^{\frac{\pi}{2}}  \left[ h_{\ell}(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, \ell} \chi_{[\beta_{i-1}, \beta_{i}]} \right] \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} \right) \\
%      &= \sign \left( \sum_{i=1}^{k} \left(p \alpha_{i, 1} - (1-p) \alpha_{i, -1} + O(\epsilon)\right) \int_{\beta_{i-1}}^{\beta_{i}} \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta}  \right)
% \end{align*}
% Lastly, we define 
% $$k_{i, L}(\theta) :=  \int_{\beta_{i-1}}^{\beta_{i}} \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} ,$$
% and we note that the $k_{i, L}$ are non-negative since the integrand is necessarily non-negative, as the support is given by $x, x^{(i)} \in \mathcal{S}_+^1$. Thus, we conclude that in probability: 
% \begin{align*}
%      \lim_{n \to \infty} m_{n, L} (\theta) &= \sign \left( \sum_{i=1}^{k} (p \alpha_{i, 1} - (1-p) \alpha_{i, -1} + O(\epsilon)) k_{i, L}(\theta) \right)
% \end{align*}
% Now we observe that $\sign(p \alpha_{i, 1} - (1-p) \alpha_{i, -1})$ is $O(\epsilon)$ from the prediction of the Bayes optimal classifier for any $\theta \in [\beta_{i-1}, \beta_i]$.  In particular, given $x = (\cos\theta, \sin\theta)$ with $\theta \in [\beta_{i-1}, \beta_i]$: 
% \begin{align*}
%     m(x) &= \sign\left( pf_1(\theta) - (1-p) f_{-1}(\theta)\right) \\
%     &= \sign\left(\left(p \left(h_1(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, 1} \chi_{[\beta_{i-1}, \beta_{i}]}(\theta) \right)  - (1-p)\left(h_{-1}(\tilde{\theta}) + \sum_{i=1}^{k} \alpha_{i, -1} \chi_{[\beta_{i-1}, \beta_{i}]}(\theta) \right)\right) \right) \\
%     &= \sign\left( p h_1(\tilde{\theta}) - (1-p) h_{-1}(\tilde{\theta})  + p \alpha_{i, 1} - (1-p) \alpha_{i, -1} \right) \\
%     &= \sign\left( O(\epsilon)  + p \alpha_{i, 1} - (1-p) \alpha_{i, -1} \right)
% \end{align*}

% Hence, if as $L \to \infty$, the $k_{i, L}(\theta)$ are functions that diverge only on $[\beta_{i-1}, \beta_i]$, then predictions given by $m_{n, L}(\theta)$ will match the predictions of the Bayes optimal classifier in probability.  Suppose that $\beta_{i-1} > 0$ and $\theta \in [\beta_{i-1}, \beta_i]$. Then, we have:
% \begin{align*}
%     k_{i, L}(\theta) &=  \int_{\beta_{i-1}}^{\beta_{i}} \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta}  \\ 
%     &\geq \int_{\theta - \epsilon}^{\theta} \psi_L(\cos(\theta - \tilde{\theta})) d \tilde{\theta} ~~ \text{for $\epsilon$ such that $\cos(\theta - \tilde{\theta})$ is monotonic.}\\
%     &= \int_{\cos(\epsilon)}^{1} \frac{\psi(u)}{\sqrt{1-u^2}} du \\ 
%     &= \int_{\cos(\epsilon)}^{1} \frac{u}{\sqrt{1 - u^2 + h(L)}\sqrt{1-u^2}} \\
%     &\geq \int_{\cos(\epsilon)}^{1} \frac{u}{1 - u^2 + h(L)} \\
%     &= -\frac{1}{2} \ln | 1 - u^2 + h(L)| \biggr\rvert_{\cos(\epsilon)}^{1}\\
%     &= - \frac{1}{2} \ln | h(L)| +  \frac{1}{2} \ln | \sin(\epsilon) + h(L)|
% \end{align*}
% As $\sin(\epsilon) > 0$, we conclude that $\lim_{L \to \infty} \left( - \frac{1}{2} \ln | h(L)| +  \frac{1}{2} \ln | \sin(\epsilon) + h(L)|\right) = \infty$.  Hence, we conclude that the $\lim_{L \to \infty} k_{i, L} = \infty$ if  $\theta \in [\beta_{i-1}, \beta_i]$.  The case for $\beta_i = 0$ follows from instead restricting to the interval $[\theta, \theta + \epsilon]$, and so, we conclude that $\lim_{L \to \infty} \lim_{n \to \infty} m_{n, L}(x) = m(x)$ in probability.  \textcolor{red}{Adit: Technically, we need to assume that the argument of the sign function is nonzero and then take $L$ large enough such that the $k_{i, L}$ term dominates and then conclude the result.}





\subsection*{Infinite Depth NNGP Kernels are Singular Kernel Smoothers}
\textcolor{red}{We first establish conditions on the dual activation under which the NNGP kernel approaches an averaging kernel with sufficiently large depth.}

\begin{theorem}
\label{thm: NNGP averaging kernel} 
Let $\Sigma^{(L)}: [-1, 1] \to \mathbb{R}$ denote the NNGP kernel of a depth $L$, fully connected network with normalized activation $\phi$.  Let $(X, y) \in \mathcal{S}^{d-1 \times n} \times \mathbb{R}^{d_o \times n}$ denote a set of $n$ linearly independent training examples and labels.  Suppose $\check{\phi}$ has a unique attractor at $0$.  Then for any $\epsilon > 0$, there exists $L_0$ such that for $L > L_0$, 
\begin{align*}
    \left|y \Sigma^{(L)}(X, x) - y {\Sigma^{(L)}}^{-1}\Sigma^{(L)}(X, x) \right| < \epsilon
\end{align*}
\end{theorem}

\begin{proof}
Since, $0$ is the unique attractor of $\check{\phi}$, we must have for any $\lim_{L \to \infty} \check{\phi}^{(L)}(\xi) = 0$ for $\xi \in \mathbb{R}$ such that $\check{\phi}(\xi) \neq \xi$.  Hence since $n$ is finite, for any $h > 0$, there exists an $L_0$ such that for $L > L_0$: 
\begin{align*}
    1 - h n^2 \leq \|\Sigma^{(L)}(X, X)\|_2 \leq 1 + h n^2
\end{align*}
Hence, we have: 
\begin{align*}
    \left| y \Sigma^{(L)}(X, x) - y {\Sigma^{(L)}}^{-1}\Sigma^{(L)}(X, x) \right| &\leq \left\|y \right\| \left\| \Sigma^{(L)}(X, x) \right\| \left\| I - {\Sigma^{(L)}}^{-1} \right\| \leq n \left( 1 - \frac{1}{1 + h n^2}\right) 
\end{align*}
Taking $h = \frac{n - \epsilon}{n}$ gives the result.  
% Taking $h = \left(\frac{1}{1 - \frac{\epsilon}{n}} - 1\right) \frac{1}{n^2}$ gives the desired result.  
\end{proof}

\textcolor{red}{We then provide examples of activation functions satisfying the above conditions.}



\textbf{Remarks.}  The conditions of Theorem \ref{thm: NNGP averaging kernel} are satisfied for $\phi(x) = \sqrt{\frac{2e}{e^2 - 1}} \sin(x) $ and for $\phi(x) = \sqrt{\frac{1}{\arcsin{2/3}}} \erf(x)$.  Note that this condition is not true for ReLU or LeakyReLU and this gives rise to a significantly different infinite depth limit.  


\textcolor{red}{We then show that the infinite depth limit of such kernels has the following singularity property.}

\begin{prop}
\label{prop: Convergence of NNGP Ratio}
Let $\Sigma^{(L)}(\xi)$ denote the NNGP kernel of a depth $L$ network with normalized activation $\phi$. Suppose there exist $A, B\in \mathbb{R}$ with $B < 1$ such that $B\xi \leq \check{\phi}(\xi) \leq B(\xi + A\xi^2)$ for $\xi \in [0, 1]$.  Then, for any $\xi \in (0, 1)$ and any fixed $\epsilon \in (0,1)$, there exists $\psi: (0, 1) \to \mathbb{R}_+$ with $\lim_{\xi \to 1} \psi(\xi) = \infty$ such that:
\begin{align*}
    \frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)} < \frac{\xi}{\epsilon} \psi(\xi)
\end{align*}
\end{prop}
\begin{proof}
We have:
\begin{align*}
    \frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)} = \frac{\check{\phi} (\Sigma^{(L-1)}(\xi)) }{\check{\phi}(\Sigma^{(L-1)}(\epsilon))} \leq \frac{\Sigma^{(L-1)}(\xi) + A  (\Sigma^{(L-1)}(\xi))^2 }{\Sigma^{(L-1)}(\epsilon)} \leq \frac{\Sigma^{(L-1)}(\xi)}{\Sigma^{(L-1)}(\epsilon)} \left[ 1 + A \Sigma^{(L-1)}(\xi)\right]
\end{align*}
Therefore, starting with $\Sigma^{(0)}(\xi) = \xi$, we have: 
\begin{align*}
     \frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)} \leq \frac{\xi}{\epsilon} \prod_{i=0}^{L-1} \left[ 1 + A \Sigma^{(i)}(\xi)\right] \leq \frac{\xi}{\epsilon} \prod_{i=0}^{\infty} \left[ 1 + A \Sigma^{(i)}(\xi)\right]
\end{align*}
Now by \cite[Ch. 5, Proposition 3.1]{SteinComplexAnalysis}, the product on the right hand side converges iff $\sum_{i=0}^{\infty}|A \Sigma^{(i)}\xi|$ converges.  By the ratio test, we have: 
\begin{align*}
    \lim_{i \to \infty} \left|\frac{\Sigma^{(i)}(\xi)}{\Sigma^{(i-1)}(\xi)} \right| = \lim_{\xi \to 0} \frac{\check{\phi}(\xi)}{\xi} \leq \lim_{\xi \to 0} \frac{B (\xi + A \xi^2)}{\xi} = B < 1
\end{align*}
Hence, the series converges and so the product converges to a value, which we denote $\psi(\xi)$.  For $\xi = 1$, we have $\Sigma^{(L)}(\xi) = 1$ and so for any $\epsilon < 1$, $\lim_{L \to \infty}  \frac{\Sigma^{(L)}(1)}{\Sigma^{(L)}(\epsilon)} = \infty$.  Hence, we conclude that $\lim_{\xi \to 1} \psi(\xi) = \infty$.  
\end{proof}

\textcolor{red}{Again all the properties above hold for sine and erf activation functions.}

\begin{example}
If $\phi(x) = \sqrt{C}\sin(x) $ for $C = \frac{2e}{e^2 - 1} < 1$, then $\check{\phi}(\xi) = C \sinh(\xi)$.  Hence, $C\xi \leq \check{\phi}(\xi) \leq C(\xi + 2\xi^2)$. 
\end{example}

\begin{example}
If $\phi(x) = \sqrt{C} \erf(x)$ for $C = \frac{1}{\arcsin(\frac{2}{3})}$, then $\check{\phi}(\xi) = C \arcsin(\frac{2\xi}{3})$.  Hence, $\frac{2}{3}C x < \check{\phi}(\xi) \leq \frac{2}{3}C (\xi + 2 \xi^2)$.  
\end{example}

\textcolor{red}{We next show that the NNGP kernel converges exponentially in the depth to a smoothing kernel estimator.}

\begin{theorem}
\label{thm: exponential convergence of NNGP}
Let $\Sigma^{(L)}(\xi)$ denote the NNGP kernel of a depth $L$ network with normalized activation $\phi$. Suppose $\check{\phi}$ has a unique attractor at $0$ and that $\check{\phi}(\xi) = C g(A \xi)$ for constants $C, A \in \mathbb{R}$ satisfying $CA < 1$ and $A \leq 1$.  Lastly, suppose $\check{\phi}(\xi) \geq C A \xi$. Then, for $\xi \in (0, 1)$,
\begin{align*}
    C^L (g'(0)A)^{L-1} g(A \xi) \leq \Sigma^{(L)}(\xi) = (CA)^{L} \xi \psi_L(\xi) ~;
\end{align*}
for analytic $\psi_L(\xi): (0, 1) \to \mathbb{R}$ that are pointwise bounded by $\psi(\xi)$ for $\psi: (0,1) \to \mathbb{R}$ with $\lim_{\xi \to 1} \psi(\xi) = \infty$.  
\end{theorem}

\begin{proof}
We begin with the upper bound.  Let $M[f]$ denote the Carleman matrix for the function $f$, i.e. for $j, k \in \mathbb{N}$, $M[f]_{j,k} = \frac{1}{k!}\left[\frac{d^k (f(x)^j)}{dx^k} \right]\vert_{x = 0}$.  \textcolor{red}{(TODO Citation)} $M[f]$ has the following properties: 
\begin{enumerate}
    \item $M[f^{(L)}] = M[f]^L$, where $f^{(L)}(x) = f(f\ldots f(x))$ denotes composition by $f$ $L$ times.
    \item $\langle M[f^{(L)}]_{1, :}^T , [1, \xi, \xi^2, \ldots ]^T \rangle = f^{(L)}(\xi)$.  
\end{enumerate} 
In particular, when $f(x) = \sum_{n=1}^{\infty} a_n x^n$, $M[f]$ is an upper triangular matrix and so $M[f^{(L)}]$ is upper triangular for all $L$.  Note that $\check{\phi}(0) = 0$ by the attractor condition and so necessarily $M[\check{\phi}]$ is upper triangular.  The NNGP kernel at depth $L$ is given by the inner product between the first row of $M[\check{\phi}^{(L)}]$, which we denote $M[\check{\phi}^{(L)}]_{1, :}$, and $Z = [1, \xi, \xi^2, \ldots]$.  Since $M[f^{(L)}] = M[f]^L$, and since $M[f^{(L)}]$ is upper triangular, we have: 
\begin{align*}
    M[\check{\phi}^{(L)}]_{1,k} &= \sum_{i=1}^{k} M[\check{\phi}^{(L-1)}]_{1,i} M[\check{\phi}]_{i,k} \\
    &= \sum_{i=1}^{k} M[\check{\phi}^{(L-1)}]_{1,i} C A \gamma_{i,k}\\
    &= CA \sum_{i=1}^{k} M[\check{\phi}^{(L-1)}]_{1,i} \gamma_{i,k} ~;
\end{align*}
for some $\gamma_{i,k} \in \mathbb{R}$. Hence by induction, we have $M[\check{\phi}^{(L)}]_{1,k} = C^L A^L \beta_{k}(L)$ for some $\beta_k(L)$, which is a function of $L$. Therefore, we conclude: 
\begin{align*}
\Sigma^{(L)}(\xi) &= \langle M[\check{\phi}^{(L)}]_{1, :}^T , [1, \xi, \xi^2, \ldots ]^T \rangle \\
&= C^L A^L \sum_{i=1}^{\infty} \beta_i(L) \xi^{i} \\
&= C^L A^L \xi \sum_{i=0}^{\infty} \beta_{i+1}(L) \xi^{i}
\end{align*}
Hence, we have
\begin{align*}
    \frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)}  \leq \frac{\xi \sum_{i=0}^{\infty} \beta_{i+1}(L) \xi^{i}}{\epsilon } 
\end{align*}
Lastly, we know from Proposition \ref{prop: Convergence of NNGP Ratio} that $\frac{\Sigma^{(L)}(\xi)}{\Sigma^{(L)}(\epsilon)}$ converges.  Therefore, the coefficients $\beta_{i+1}(L)$ cannot diverge with $L$ and we conclude that:
$$ \Sigma^{(L)}(\xi) = (CA)^{L} \xi  \sum_{i=0}^{\infty} \beta_{i+1} \xi^{i} ~; $$
for $\{\beta_{j}\}_{j=1}^{\infty} \subset \mathbb{R}$ are independent of $\xi$.  Hence, we let $\psi_L(\xi) = \sum_{i=0}^{\infty} \beta_{i+1} \xi^{i}$, and since the $\beta_{i+1}$ do not diverge with $L$, we necessarily have that the functions are bounded above by some $\psi(\xi)$.  

Next, we prove the lower bound.  This again follows from an analysis of the terms of $M[\check{\phi}^{(L)}]_{1, :}$.  In particular, letting $[f]_k$ denote the $k^{th}$ coefficient of the Maclaurin series of $f$, we have 
$$M[\check{\phi}^{(L)}]_{1,k} \geq [\check{\phi}]_1^{L-1} [\check{\phi}]_k = (CAg'(0))^{L-1}  C \frac{d^k g}{dx^k}\left(0 \right) A^k . $$
Hence, by taking the inner product with the vector $[1, \xi, \xi^2, \ldots]$, we have that $\check{\phi}^{(L)}(\xi) \geq C^L (Ag'(0))^{L-1}) g(A \xi)$.  
\end{proof}

Again, the normalized activations for sine and erf satisfy the above conditions.  In particular, $C = \frac{2e}{e^2-1}, A = 1$ for the normalized sine activation and $C = \frac{1}{\arcsin(\frac{2}{3})}, A = \frac{2}{3}$ for the normalized $\erf$ activation.  Moreover, we have the following corollary.  

\begin{corollary}
For neural networks with normalized sine or erf activations and for $\xi \in (0, 1)$, the corresponding NNGP kernel of depth $L$ satisfies:
\begin{align}
    \Sigma^{(L)}(\xi) = (CA)^{L} \xi  \sum_{i=0}^{\infty} \beta_{2i+1} \xi^{2i} ~;
\end{align}
for constants $\{\beta_{2i+1}\}_{i=0}^{\infty}$ satisfying $\lim_{L \to \infty} \beta_{2i+1} < \infty$.  
\end{corollary}
\begin{proof}
The proof follows from a combinatorial argument. In particular, since the Taylor series expansions of the corresponding dual activations have no even powers, $M[\check{\phi}]_{jk}$ is nonzero iff the integer $k$ can be partitioned into $j$ blocks with only odd integers.  This is impossible when $j$ and $k$ have differing parity.  Hence, we conclude that $M[\check{\phi}]_{1, :} M[\check{\phi}]_{:, k} = 0$ whenever $k$ is even.  Hence, by induction, $M[\Sigma^{(L)}]_{1, k} = 0$ for all even $k$.  
\end{proof}

\textbf{Remarks.}  Empirically, for the normalized sine activation, we observe the stronger statement that the $\beta_{2i+1} \leq 1$ and in particular, we observe that $\Sigma^{(L)}(\xi) \leq (C)^{L} \frac{\xi}{1 - \xi^2}$ for $C = \frac{2e}{e^2-1}$.  As we show in the experiments section, this approximation is within 1\% of the performance of the deep NNGP for networks with the normalized sine activation.   

\subsection*{Infinite Depth NTKs are Singular Kernel Smoothers}
\textcolor{red}{We next establish conditions on the dual activation and its derivative such that the NTK kernel approaches a kernel smoother with sufficiently large depth. Note that the convergence is still exponential for the NTK. }

\begin{theorem}
\label{thm: NTK convergence to smoother}
Let $K^{L}: [-1, 1] \to \mathbb{R}$ denote the NTK of a depth $L$, fully connected network with normalized activation $\phi$.  Suppose that $\check{\phi}$ has a unique attractor at $0$ and that $\check{\phi}(\xi) = Cg(A\xi)$ for constants $C, A \in \mathbb{R}$ with $CA < 1$ and $A \leq 1$.  Suppose that $CA \leq \check{\phi}'(\xi) \leq CA(1 + B\xi^2)$ for $B \in \mathbb{R}$ for $\xi \in [0,1]$.  Let $(CA)^L \xi \leq \Sigma^{(L)}(\xi) \leq (CA)^L \xi \psi(\xi)$ as given by Theorem \ref{thm: exponential convergence of NNGP}.  Then for $\xi \in (0, 1)$, 
\begin{align*}
    (CA)^L \xi (1 + L) \leq K^{(L)}(\xi) <  (CA)^L e^{\frac{B\xi\psi(\xi)}{1 - CA}} \xi \left( 1 + \psi(\xi) L \right)  ~;
\end{align*}
and $\lim_{L \to \infty} K^{(L)}(1) = \infty$ if $\check{\phi}'(1) \geq 1$.  
\end{theorem}

\begin{proof}
The proof follows from that of Theorem \ref{thm: exponential convergence of NNGP} and the recursive formula for the NTK.  In particular, we have: 
\begin{align*}
    K^{(L)}(\xi) = K^{(L-1)}(\xi) \check{\phi}'(\Sigma^{(L-1)}(\xi)) + \Sigma^{(L)}(\xi) ~;~ K^{(0)}(\xi) = \xi
\end{align*} 
Unwinding the recursion, we have: 
\begin{align*}
    K^{(L)}(\xi) &= \xi \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] + \sum_{i=1}^{L} \left[ \Sigma^{(i)}(\xi) \prod_{j=i}^{L-1} \check{\phi}'(\Sigma^{(j)}(\xi))\right] \\
\end{align*}
    % &\leq \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] \left( \xi + \sum_{i=1}^{L} \Sigma^{(i)}(\xi) \right) ~~ \text{\textcolor{red}{TODO justification with convexity of dual}} \\
    % &\leq h(L) \left( \xi + \sum_{i=1}^{L} (CA)^i \xi \psi(\xi) \right) \\
    % &\leq h(L) \xi \left( 1 + \psi(\xi) \frac{1}{1 - CA}\right)
We now establish the upper bound.  Namely, using the assumption on $\Sigma^{(L)}(\xi)$ and the upper bound on $\check{\phi}'$, we have: 
\begin{align*}
    K^{(L)}(\xi) &= \xi \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] + \sum_{i=1}^{L} \left[ \Sigma^{(i)}(\xi) \prod_{j=i}^{L-1} \check{\phi}'(\Sigma^{(j)}(\xi))\right] \\
    &\leq \xi \left[\prod_{i=0}^{L-1} CA (1 + B (CA)^i \xi \psi(\xi)) \right] + \sum_{i=1}^{L} \left[ (CA)^i \xi \psi(\xi) \prod_{j=i}^{L-1} CA (1 + B (CA)^j \xi \psi(\xi))\right] \\
    &\leq \xi (CA)^L \left[\prod_{i=0}^{L-1}  e^{B (CA)^i \xi \psi(\xi)} \right] + \sum_{i=1}^{L} \left[ (CA)^i \xi \psi(\xi) (CA)^{L-i} \prod_{j=i}^{L-1}  e^{B (CA)^j \xi \psi(\xi)}\right] \\
    &\leq  \xi (CA)^L  e^{\frac{B \xi \psi(\xi)}{1-CA}}  + \sum_{i=1}^{L}  (CA)^L \xi \psi(\xi) e^{\frac{B \xi \psi(\xi)}{1-CA}} \\
    &\leq (CA)^L \xi e^{\frac{B \xi \psi(\xi)}{1-CA}} (1 + \psi(\xi)L )
\end{align*}

We similarly establish the lower bound.  
\begin{align*}
     K^{(L)}(\xi) &= \xi \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] + \sum_{i=1}^{L} \left[ \Sigma^{(i)}(\xi) \prod_{j=i}^{L-1} \check{\phi}'(\Sigma^{(j)}(\xi))\right] \\
     &\geq \xi \left[\prod_{i=0}^{L-1} CA \right] + \sum_{i=1}^{L} \left[ (CA)^i \xi \prod_{j=i}^{L-1} CA \right]\\
     &\geq \xi (CA)^L + \sum_{i=1}^{L} (CA)^L \xi \\
     &\geq \xi (CA)^L (1 + L)
\end{align*}

% The first inequality above follows from the fact that the dual activation is convex and non-decreasing on $[0, 1]$, and the fact that the derivative of a dual activation is itself a dual activation (without normalization by a constant factor).  Now, we analyze the convergence of the term $h(L) = \prod_{i=0}^{L} \check{\phi}'(\Sigma^{(i)}(\xi))$ as $L \to \infty$. The attractor condition on $\check{\phi}$ implies $\check{\phi}'(0) < 1$ and $\lim_{L \to \infty} \Sigma^{(L)}(\xi) = 0$.  Hence, there exists $L_0$ such that for $L > L_0$, $\check{\phi}'(\Sigma^{(L)}(\xi)) < 1$.  Therefore, $\lim_{L \to \infty} h(L) = 0$, which completes the proof of the upper bound.  
Lastly, we have that $K^{(L)}(1) = K^{(L-1)}(1) \check{\phi}'(1) + 1$, which must diverge (at least at rate $O(L)$) if $\check{\phi}'(1) \geq 1$.  
\end{proof}
\textcolor{red}{Naturally, the two activations we have considered throughout this work again satisfy all of the conditions of this theorem.   }

The following corollary connects the bound of the NNGP with that of the NTK.  In particular, as depth approaches infinity, the NTK has at most an extra exponential factor in $\xi \psi(\xi)$ on top of the bound of the NNGP. 
\begin{corollary}
Under the setting of Theorem \ref{thm: NTK convergence to smoother}, for any $\xi \in (0, 1)$ and any fixed $\epsilon \in (0,1)$: 
\begin{align*}
    \frac{\xi}{\epsilon} \frac{1}{\psi(\epsilon)} e^{-\frac{B \epsilon \psi(\epsilon)}{1-CA}}  \leq \lim_{L \to \infty} \frac{K^{(L)}(\xi)}{K^{(L)}(\epsilon)} \leq \frac{\xi}{\epsilon} \psi(\xi) e^{\frac{B \xi \psi(\xi)}{1-CA}} 
\end{align*}
\end{corollary}
% Under additional assumptions on the dual activation, the NTK also approaches a kernel smoother exponentially in the depth.  

% \begin{corollary}
%     Under the setting of Theorem \ref{thm: NTK convergence to smoother}, suppose that $\check{\phi}'(\xi) \leq CA(1 + B\xi^2)$ for $B \in \mathbb{R}$. Then, 
%     \begin{align*}
%             K^{(L)}(\xi) <  (CA)^L e^{\frac{B\xi}{1 - CA}} \xi \left( 1 + \psi(\xi) \frac{1}{1 - AC} \right)
%     \end{align*}
% \end{corollary}
% \begin{proof}
% Following the proof of Theorem \ref{thm: NTK convergence to smoother}, we have: 
% \begin{align*}
%     h(L) &=  \left[\prod_{i=0}^{L-1} \check{\phi}'(\Sigma^{(i)}(\xi))\right] \\
%          &\leq \left[\prod_{i=0}^{L-1} \check{\phi}'(\xi (CA)^{i} \psi(\xi))\right] \\
%          &\leq \left[\prod_{i=0}^{L-1} CA (1 + B \xi (CA)^{i} \psi(\xi)) \right] \\
%          &\leq (CA)^L \left[\prod_{i=0}^{L-1}e^{B \xi (CA)^{i} \psi(\xi)} \right] \\
%          &\leq (CA)^L \exp\left(\sum_{i=0}^{\infty} B \xi (CA)^{i} \psi(\xi) \right) \\
%          &= (CA)^L \exp\left(\frac{B \xi\psi(\xi)}{1 - CA} \right)
% \end{align*}
% Hence, substituting into the result of Theorem \ref{thm: NTK convergence to smoother}, we conclude:
%     \begin{align*}
%             K^{(L)}(\xi) <  (CA)^L e^{\frac{B\xi}{1 - CA}} \xi \left( 1 + \psi(\xi) \frac{1}{1 - AC} \right)
%     \end{align*}
% \end{proof}


\subsection*{Infinite Depth ReLU NNGP Kernel and NTK}
\textcolor{blue}{Adit: Write out how the NNGP Kernel converges to the all 1's kernel and that the NTK for ReLU converges to a kernel that averages all class labels as the prediction.}



\section{Old Pole Order Analysis}
We now prove the result for the case where $\check{\phi}$ is replaced by a piece-wise linear function around $\xi = 0$ and $\xi = 1$.

\begin{lemma}
\label{lemma: piecewise linear NTK}
Let 
\begin{align*}
f(x) = \begin{cases} a x ~~ \text{if $x \in [0, c)$}  \\ g(x) ~~ \text{if $x \in [c, d)$} \\ 1 - b(1 - x) ~~ \text{if $x \in [d, 1]$}   \end{cases} ~~, ~~ h(x) = \begin{cases} a  ~~ \text{if $x \in [0, c]$}  \\ g'(x) ~~ \text{if $x \in (c, d)$} \\ b ~~ \text{if $x \in [d, 1]$}   \end{cases}  ~;
\end{align*}
such that $f(x)$ is strictly monotonically increasing and where $g(x)$ can be written as a convergent power series with non-negative coefficients and $0 < a < 1$ and $b > 1$.  For $L \geq 1 $, let 
$$k^{(L)}(x) = k^{(L-1)}(x) h(f^{(L-1)}(x)) + f^{(L)}(x)  ~~; ~~ k^{(0)}(x) = x. $$  
Then for $x \in (d, 1]$:
$$\lim_{L \to \infty} \frac{k^{(L)}(x)}{a^{L} (L + 1)} = \frac{R(x)}{(1 - x)^{-\log_b a}} ~~;$$
where $R(x)$ is bounded on $[0, 1]$.  
\end{lemma}
\begin{proof}
We consider the case of continuous $L$ (i.e. the flow instead of the discrete dynamical system).  In particular, as $0$ is the unique fixed point attractor of $f(x)$, we have for $x \in (d, 1)$ that after $L_0(x)$ time steps, $f^{(L_0(x))}(x) = f(d)$ and after $L_1$ time steps, $f^{(L_1)}(d) = f(c)$.   For any $L > L_0(x) + L_1$, we then have that $f^{(L)}(x) = a^{L - L_0(x) - L_1} f(c)$.  Hence there exists constant $x_0 > 0$ such that for $x \in (d, 1)$: 
\begin{align*}
    \lim_{L \to \infty}  \frac{a^{L - \lceil L_0(x) \rceil} f(x_0)}{a^L} \leq \lim_{L \to \infty} \frac{f^{(L)}(x)}{a^L} \leq \lim_{L \to \infty}  \frac{a^{L - L_0(x) - L_1} f(c)}{a^L} .
\end{align*}
Lastly, we can compute $L_0(x)$ by solving: 
\begin{align*}
    1 - b^{L_0(x)}(1 - x) = f(d) \implies L_0(x) = \log_a \left( \frac{1 - x}{1 - f(d)} \right)^{- \log_b a}
\end{align*}
Therefore, as $\lceil L_0(x) \rceil \geq L_0(x) - 1$, 
\begin{align*}
      \frac{af(x_0)}{ (1 - x)^{- \log_b a}} \leq \lim_{L \to \infty} \frac{f^{(L)}(x)}{a^L} \leq \frac{(1 - f(d))^{- \log_b a} f(c) }{a^{L_1} (1 - x)^{- \log_b a}} =  \frac{C}{ (1 - x)^{- \log_b a}} ~;
\end{align*}
for some positive constant $C$. Now via a similar analysis, we note that for $L > L_0(x) + L_1$, $h(f^{(L)}(x)) = a$.  Hence, for $L = L_0(x) + L_1 + T$ steps, we have by induction: 
\begin{align*}
    k^{(L)}(x) \leq a^{T} [k^{(L_0(x) + L_1)}(x) + T f(c)] = a^{L - L_0(x) - L_1} [k^{(L_0(x) + L_1)}(x) + (L - L_0(x) - L_1) f(c)]
\end{align*}
Now select $\tilde{C}(x)$ as a lower bound on the value of $k^{(L)}$ for $L$ such that $f^{(L)}(x) < c$.  Then, there exists some $x_0 \in [0, c)$ such that by induction on $L$: 
\begin{align*}
     k^{(L)}(x) \geq  a^{L - \lceil L_0(x) \rceil} [\tilde{C}(x) + (L - L_0(x) - L_1) f(x_0)]
\end{align*}
Therefore via the upper bound on $k^{(L)}(x)$: 
\begin{align*}
    \lim\limits_{L \to \infty} \frac{k^{(L)}(x)}{a^{L}(L+1)} &\leq \lim\limits_{L \to \infty} a^{-L_0(x) - L_1} \frac{k^{(L_0(x) + L_1)}(x) + (L - L_0(x) - L_1) f(c)}{L+1} \\
    &= a^{-L_0(x) - L_1} f(c) \\
    &= \frac{C}{ (1 - x)^{- \log_b a}} .
\end{align*}
Similarly, the lower bound on $k^{(L)}(x)$ yields: 
\begin{align*}
    \lim\limits_{L \to \infty} \frac{k^{(L)}(x)}{a^{L}(L+1)} & \geq  \frac{af(x_0)}{ (1 - x)^{- \log_b a}}, 
\end{align*}
which concludes the proof of the lemma. 
\end{proof}

Our first key observation is that Lemma \ref{lemma: piecewise linear NTK} can be extended to the case where $f$ is only linear around $0$. 

\begin{lemma}
\label{lemma: two piece pole order}
Let 
\begin{align*}
f(x) = \begin{cases} a x ~~ \text{if $x \in [0, c)$}  \\ g(x) ~~ \text{if $x \in [c, 1]$}  \end{cases} ~~, ~~ h(x) = \begin{cases} a  ~~ \text{if $x \in [0, c]$}  \\ g'(x) ~~ \text{if $x \in (c, 1]$} \end{cases} ~;
\end{align*}
such that $f(x)$ is monotonically increasing and where $g(x)$ can be written as a convergent power series with non-negative coefficients satisfying $g(1) = 1$ and $0 < a < 1$.  For $L \geq 1 $, let 
$$k^{(L)}(x) = k^{(L-1)}(x) h(f^{(L-1)}(x)) + f^{(L)}(x)  ~~; ~~ k^{(0)}(x) = x. $$  
Then for $x \in (d, 1]$:
$$\lim_{L \to \infty} \frac{k^{(L)}(x)}{a^{L} (L + 1)} = \frac{R(x)}{(1 - x)^{-\log_b a}} ~~;$$
where $R(x)$ is bounded in $[0, 1]$.  
\end{lemma}

\begin{proof}
We will first show that $\lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} = \frac{Q(x)}{(1 - x)^{-\log_b a}}$ for $Q(x)$ bounded in $[0, 1]$.  As $g(x)$ can be written as a convergent power series with non-negative coefficients with $g(1) = 1$, it is convex.  Hence, we upper bound $g(x)$ by the following function that is linear around $x = 0$ and $x = 1$: 
\begin{align*}
    f_{\epsilon}(x) = \begin{cases} a x ~~ \text{if $x \in [0, c)$}  \\ g(x) ~~ \text{if $x \in [c, 1-\epsilon)$} \\ 1 - (g'(1) - \epsilon)(1 - x) ~~ \text{if $x \in [1 - \epsilon, 1]$} \end{cases}
\end{align*}
Now by Lemma \ref{lemma: piecewise linear NTK} and as $f_{\epsilon}, f$ have the same normalizing factor $a$, we have that: 
\begin{align*}
    \lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} \leq \lim\limits_{L \to \infty} \frac{f_{\epsilon}^{(L)}(x)}{a^{L}} = \frac{Q_1(x)}{(1 - x)^{-\log_{g'(1) - \epsilon} a}}
\end{align*}
As $\epsilon$ is arbitrary, we conclude that the pole of $f$ at $x = 1$ has order at most $- \log_{g'(1)} a$.  Similarly, we can lower bound $f$ via the following function: 
\begin{align*}
    \tilde{f}(x) = \begin{cases} a x ~~ \text{if $x \in [0, d)$} \\ 1 - g'(1)(1 - x) ~~ \text{if $x \in [d, 1]$} \end{cases} ~;
\end{align*}
where $d$ is the intersection point of the tangent lines of $f$ at $x = 0$ and $x = 1$.  Again Lemma \ref{lemma: piecewise linear NTK} and as $\tilde{f}, f$ have the same normalizing factor $a$, we have that: 
\begin{align*}
 \lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} \geq \lim\limits_{L \to \infty} \frac{\tilde{f}^{(L)}(x)}{a^{L}} = \frac{Q_2(x)}{(1 - x)^{-\log_{g'(1)} a}}    
\end{align*}
Therefore, we conclude that: 
\begin{align*}
    \lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} = \frac{R(x)}{(1 - x)^{-\log_{g'(1)} a}} ~;
\end{align*}
for some $R(x)$ bounded in $[0, 1]$.  Now to bound the pole order of the normalized iteration of $k$ at $x =1$, we observe that there exists $L_0$ such that for $L \geq \lceil L_0 \rceil$, $f^{(L)}(x) \leq c$.  Hence, there exists some $x_0 \in [0, c)$ such that: 
\begin{align*}
    k^{(L)}(x) = a^{L - \lceil L_0 \rceil} (\tilde{C}(x) + (L - \lceil L_0 \rceil) f(x_0))
\end{align*}
Therefore, for $x \in (c, 1)$:
\begin{align*}
    \lim\limits_{L \to \infty} \frac{k^{(L)}(x)}{a^{L}(L+1)} = f(x_0) a^{ - \lceil L_0 \rceil} = \lim\limits_{L \to \infty} \frac{f^{(L)}(x)}{a^{L}} =  \frac{R(x)}{(1 - x)^{-\log_{g'(1)} a}}, 
\end{align*}
which concludes the proof of the lemma.  
\end{proof}



We lastly need to establish a similar lower bound on the the above limit to conclude the proof.  We will construct the lower bound by first establishing the pole order of the NNGP iteration and then showing that the NNGP pole order is a lower bound on the NTK pole order.  Note that we have already established an upper bound on the pole order of the infinite depth NNGP via Eq.~\eqref{eq: NNGP approximation}.  Namely, by Eq.~\eqref{eq: NNGP approximation} and Lemma \ref{lemma: two piece pole order}: 
\begin{align*}
      \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} &= \lim_{\epsilon \to 0} \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi) - f_{\epsilon}^{(L)}(\xi)}{a^{L}} +  \lim_{\epsilon \to 0}  \lim\limits_{L \to \infty} \frac{f_{\epsilon}^{(L)}(\xi)}{a^{L}} \leq \frac{Q_1(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}} ~.
\end{align*}
Now, we alternatively lower bound $\check{\phi}$ via the following function: 
\begin{align*}
    \tilde{f}(\xi) = \begin{cases} a_1 \xi ~~ \text{if $x \in [0, c)$}  \\ 1 - \check{\phi}'(1)(1- \xi) ~~ \text{if $x \in [c, 1]$}  \end{cases} ~;
\end{align*}
where $\tilde{f}(c)$ corresponds to the intersection of the tangent lines of $\check{\phi}$ at $\xi = 0$ and $\xi = 1$.  As in the proof of Lemma \ref{lemma: two piece pole order}, we thus have that: 
\begin{align*}
    \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} \geq \lim\limits_{L \to \infty}  \frac{\tilde{f}^{(L)}(\xi)}{a^{L}} = \frac{Q_2(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}}
\end{align*}
Hence, we conclude that: 
\begin{align*}
    \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} = \frac{Q(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}} ~, 
\end{align*}
where we also know that $Q(\xi)$ can be written as a convergent power series on $[0, 1]$ with non-negative coefficients by definition of the NNGP iteration.  Lastly, we utilize Eq.~\ref{eq: Closed form for NTK} to show that: 
\begin{align*}
    \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} \leq  \lim\limits_{L \to \infty}  \frac{K^{(L)}(\xi)}{a^{L}(L+1)} ~.
\end{align*}
In particular, by Eq.~\ref{eq: Closed form for NTK}, we have: 
\begin{align*}
    K^{(L)}(\xi)= \sum_{i=0}^{L} \check{\phi}^{(i)}(\xi) \prod_{k=i}^{L-1} \check{\phi}'\left(\check{\phi}^{(k)}(\xi)\right) ~~;
\end{align*}
and we next write $\check{\phi}^{(i)}(\xi)$ as a product.  Namely, using the power series representation for $\check{\phi}$ and unrolling the iteration, we have: 
\begin{align*}
    \check{\phi}^{(i)}(\xi) &= \sum_{j=1}^{\infty} a_j \left(\check{\phi}^{(i-1)}(\xi)\right)^{j} \\
    &= a_1 \check{\phi}^{(i-1)}(\xi) \left (1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(i-1)}(\xi)\right)^{j} \right) \\
    &= a_1^{i} \xi \prod_{k=0}^{i - 1} \left( 1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j} \right) ~.
\end{align*}
We similar use the power series for $\check{\phi}'(\xi)$ to conclude: 
\begin{align*}
    \check{\phi}'\left(\check{\phi}^{(k)}(\xi)\right) &= \sum_{j=1}^{\infty} j a_j \left(\check{\phi}^{(k)}(\xi)\right)^{j-1} \\
    &\geq \sum_{j=1}^{\infty} a_j \left(\check{\phi}^{(k)}(\xi)\right)^{j-1} \\
    &\geq a_1 \left(1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j-1} \right) \\
    &\geq a_1 \left(1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j} \right) ~~ \left(\text{as $\check{\phi}^{(k)}(\xi) \leq 1$.} \right) ~. 
\end{align*}
Therefore, we simplify Eq.~\ref{eq: Closed form for NTK} as follows: 
\begin{align*}
      K^{(L)}(\xi) &= \sum_{i=0}^{L} \check{\phi}^{(i)}(\xi) \prod_{k=i}^{L-1} \check{\phi}'\left(\check{\phi}^{(k)}(\xi)\right) \\
      &\geq \sum_{i=0}^{L} a_1^{i} \xi \prod_{k=0}^{i - 1} \left( 1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j} \right) \prod_{k'=i}^{L-1} a_1 \left(1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k')}(\xi)\right)^{j} \right) \\
      &= \sum_{i=0}^{L} a_1^{i} \xi \prod_{k=0}^{L - 1} \left( 1 + \sum_{j=2}^{\infty} \frac{a_j}{a_1} \left(\check{\phi}^{(k)}(\xi)\right)^{j} \right) \\
      &= (L+1) \check{\phi}^{(L)}(\xi) ~.
\end{align*}
Therefore, we conclude: 
\begin{align*}
    \frac{K^{(L)}(\xi)}{a^{L} (L + 1)} \geq \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} ~, 
\end{align*}
and so: 
\begin{align}
\label{eq: Lower bound on normalized iterated NTK}
    \lim\limits_{L \to \infty}  \frac{K^{(L)}(\xi)}{a^{L}(L+1)} \geq \lim\limits_{L \to \infty}  \frac{\check{\phi}^{(L)}(\xi)}{a^{L}} = \frac{Q(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}}.
\end{align}
Lastly, we combine Eq.~\ref{eq: Lower bound on normalized iterated NTK} and \ref{eq: Upper bound on normalized iterated NTK} to conclude: 
\begin{align*}
   \frac{Q(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}} \leq \lim\limits_{L \to \infty}  \frac{K^{(L)}(\xi)}{a^{L}(L+1)} \leq \frac{\tilde{R}(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}}~. 
\end{align*}
Thus, by the squeeze theorem: 
\begin{align*}
    \lim\limits_{L \to \infty}  \frac{K^{(L)}(\xi)}{a^{L}(L+1)} = \frac{R(\xi)}{(1 - \xi)^{-\log_{\check{\phi}'(1)} \check{\phi}'(0)}}~, 
\end{align*}
where $R(\xi)$ is bounded and by Eq.~\ref{eq: Closed form for NTK}, can be written as a power series with non-negative coefficients.  This concludes the proof of Theorem \ref{theorem: Dynamical Systems NTK}.    



We make use of the following lemma throughout our proofs. 

\begin{lemma}
\label{lemma: limit for order of pole}
Let $f(x): [0, 1] \to \mathbb{R}$ such that $f$ has a singularity only at $x = 1$. Then $x = 1$ is a singularity of order $\alpha$ iff for any $b > 1$:  
\begin{align}
\label{eq: log order of pole}
    -\log_b \left(\lim_{\epsilon \to 0^+}  \frac{f(1 - b\epsilon)}{f(1  - \epsilon)}\right) = \alpha.
\end{align}
\end{lemma}

\begin{proof}
Note that $f$ has a singularity of order $\alpha < \infty$ iff
\begin{align*}
    f(x) = \frac{R(x)}{(1 - x)^{\alpha}},
\end{align*}
where $R(x)$ is bounded on $[0, 1]$, $R(1) \neq 0$, and $R(x)$ is continuous at $1$.  Hence,  by directly substituting the closed form for $f$ into Eq.~\eqref{eq: log order of pole}, we have that: 
\begin{align*}
    -\log_b \left(\lim_{\epsilon \to 0^+}  \frac{f(1 - b\epsilon)}{f(1  - \epsilon)}\right) &= -\log_b \left(\lim_{\epsilon \to 0} \frac{R(1 - b\epsilon)}{R(1 - \epsilon)} b^{-\alpha} \right) = \alpha ~.
\end{align*}
If the pole has infinite order, then we necessarily have: 
\begin{align*}
    \lim_{\epsilon \to 0^+}  \frac{f(1 - b\epsilon)}{f(1  - \epsilon)} = 0 ~, 
\end{align*}
and so $\alpha = -\log_b(0) = \infty$.  The other direction follows by a similar line of reasoning.  In particular, suppose there exists $\alpha < \infty$ such that 
\begin{align*}
    -\log_b \left(\lim_{\epsilon \to 0^+}  \frac{f(1 - b\epsilon)}{f(1  - \epsilon)}\right) = \alpha.
\end{align*}
Then, as $f(x)$ has a singularity at $x = 1$, there exists $\beta < \infty$ such that
\begin{align*}
    f(x) = \frac{R(x)}{(1 - x)^{\beta}}~,
\end{align*}
where $R(x)$ is bounded on $[0, 1]$, $R(1) \neq 0$, and $R(x)$ is continuous at $1$.  We then conclude that $\beta = \alpha$.  
\end{proof}




















